Sibyl: Forecasting Time-Evolving Query Workloads

Database systems often rely on historical query traces to perform workload-based performance tuning. However, real production workloads are time-evolving, making historical queries ineffective for optimizing future workloads. To address this challenge, we propose SIBYL, an end-to-end machine learning-based framework that accurately forecasts a sequence of future queries, with the entire query statements, in various prediction windows. Drawing insights from real-workloads, we propose template-based featurization techniques and develop a stacked-LSTM with an encoder-decoder architecture for accurate forecasting of query workloads. We also develop techniques to improve forecasting accuracy over large prediction windows and achieve high scalability over large workloads with high variability in arrival rates of queries. Finally, we propose techniques to handle workload drifts. Our evaluation on four real workloads demonstrates that SIBYL can forecast workloads with an $87.3\%$ median F1 score, and can result in $1.7\times$ and $1.3\times$ performance improvement when applied to materialized view selection and index selection applications, respectively.

==> backup_content/1.introduction.vldb.tex <==
\vspace{-2mm}
\section{Introduction}
%\yuanyuan{@Hanxian, please go over all figures to make sure that the workload names have been changed to the ones we are currently using. e.g. Figure 9 is still using the old names for sigmod submission.}

%\yuanyuan{@Hanxian, a high level question. I am always unsure when to use LSTM and when to use LSTMs. LSTM is for a single layer model, right? So, if we say stacked LSTMs, we should use LSTMs, right? Can you make sure the usage is consistent thoughout the paper?}
%\hanxian{TODO: check LSTM"s"}
\begin{comment}
Optimization techniques in DBMSs such as view selection~\cite{mami2012survey,zhou2006dynamic}, query results caching~\cite{DBLP:conf/vldb/DarFJST96}, index recommendation~\cite{gani2016survey, das2019automatically}, partitioning~\cite{agrawal2004integrating,curino2010schism}, \etc usually assume workloads are static. With the rapid development of today's data-driven applications and the growing complexity of big data, conventional techniques with the static workload assumption are sub-optimal. We demonstrate the importance of workload forecasting with view selection as a motivation application:

%\jcr{I think we could elaborate a bit more in the following example by using a few (couple) filter conditions, each one with different characteristics, to showcase that it is not as simple as assuming that everything is a sliding time window}
\textsc{Example 1.} A workload recurrently queries the last week's data and a high frequent query's filter on Jan 25th is
\colorbox{gray!20}{WHERE event\_date}\\ \colorbox{gray!20}{>= Jan 18th  AND event\_date <= Jan 25th}. The values of predicates `event\_date >=' and `event\_date <=' in the WHERE clause are changing upon query arrival time. They are `Jan 18th' AND `Jan 25th' on Jan 25th's queries while changing to `event\_date >= Jan 19th AND event\_date <= Jan 26th' in Jan 26th's queries, etc. 

The conventional view selection techniques (\eg~\cite{zhou2006dynamic}) assume workloads are static and select views based on statistics of the historical queries, \eg the high frequent historical query with filter predicates `event\_date >= Jan 22 AND event\_date <= Jan 29'. The materialized views based on the historical predicate values cannot answer the future query since the real values are changing over query time, which leads to a sub-optimal solution. 
%view selection example is shown in Figure~\ref{fig:moti}: conventional view recommendation ~\cite{zhou2006dynamic} assumes the workload is static and materializes highly frequent historical queries, but fails to capture the workload evolving features. 
The optimal materialization results are hard to derive by only considering the highly frequent historical queries while ignoring the time-evolving nature of the workloads. This calls for a new forecasting technique that captures the time-evolving characteristics of the workloads in a long-time horizon and forecasts the future workloads precisely. 

% \begin{comment}
% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=\linewidth]{figure/example2.pdf}
%   \caption{Motivation example. Conventional view selection assumes the workload is static and materializes the result of historical query, which fails to answer the future query. With \sys, view selection is performed based on the forecasted workload and improve \todox{$xxx\times$} performance.
%   \hanxian{seems too much texts in the figure? should I separate the example with the SIBYL workflow?}}
%   \label{fig:moti}
% \end{figure}
 \end{comment}


%\jcr{Consider introducing this paragraph (how useful can forecasting be) before talking about the example and the complexity of doing it right.}
\begin{comment}
Moreover, forecasting future query statements as well as their corresponding arrival time before they really arrive benefits DBMS in many aspects. By predicting the future queries that will arrive in the next forecasting interval, DBMS is allowed to speculatively execute the queries and skip the execution when the actual future queries arrive, thereby improving performance. Workload forecasting also helps auto-tuning the DMBS ahead of time: forecasting the possible values of constants in selection (or join) predicates can help DBMS create indexes and views; forecasting the future query as well as the arrival time give valuable hints to perform better auto-scaling; forecasting the set of tables and attributes in predicates allows DBMS to construct partial or full query plan ahead of time; forecasting the sort (ORDER BY) and aggregate (COUNT) operator to help DBMS in pre-allocation of buffer pages and configuring \# CPU-bound threads to parallelize the execution, etc. %\hanxian{Need help here to elaborate the potential benefit of our framework. And why predicting a sequence of queries + arrival time is critical. What \sys\ can do but other works cannot do, e.g., VM?} \textcolor{gray}{COPY-PASTE from TODS'21 paper: If we can predict the next SQL query in its entirety during the user think time, then we can speculatively execute it and prefetch its results into the memory. When the actual next query arrives, we can skip its execution and return the prefetched results directly from the memory. Even if an SQL query cannot be predicted in its entirety, knowing apriori the impending query operators and their associated schema elements (defined as query fragments) from the successive query is useful. If we know the set of tables and attributes participating in projection/selection/join/aggregate predicates, then it can allow for partial or full query plan construction during the user think time. The database can also evaluate it partially or entirely depending on the structure of the SQL query. Predicting sort (ORDER BY) and aggregate (COUNT) operator fragments can help in pre-allocation of buffer pages and configuring \# CPU-bound threads to parallelize their execution. Likewise, being cognizant of the selection (or join) predicates can help us pre-load or create indexes if we know the possible range of constants in the selection predicates.}
\end{comment}

Workload-based optimization is a critical aspect of database management, which tunes a database management system (DBMS) to maximize its performance for a specific workload. 
%It is essential to ensure that database systems can efficiently handle the demands of modern applications. 
Consequently, a large number of performance tuning tools have been developed for workload-based optimization. 
While execution statistics may be sufficient for optimizing certain aspects of the system (e.g., buffer pool size), many optimizations require an understanding of semantics of the queries, necessitating a workload query trace as input.
%While workload metrics, such as resource utilization and runtime statistics, may be sufficient for optimizing certain aspects of the system with some of these tools, other workload optimization tools require an understanding of the semantics of queries in the workload, making a workload query trace necessary as input.
For instance, many commercial database products~\cite{sqlserver,db2,oracle,informix} support physical design tools 
%provided by many established commercial database products~\cite{sqlserver,db2,oracle,informix}, 
such as Microsoft's AutoAdminn~\cite{autoadmin} and IBM's DB2 design advisor~\cite{db2advisor}. 
%have been developed. 
These tools automatically recommend physical design features, such as indexes, materialized views, partitioning schemes of tables, and multidimensional clustering (MDC)~\cite{mdc} of tables for a given workload of queries. Another related workload-based optimization technique is semantic 
caching~\cite{DBLP:conf/sigmod/StonebrakerJGP90,DBLP:conf/edbt/ChenR94a,DBLP:conf/vldb/DarFJST96,DBLP:journals/pvldb/DurnerCL21}, which involves caching frequently accessed query results based on the semantic meaning of the queries to accelerate repeated execution. In fact, many of the aforementioned workload-based optimization techniques form the foundational pieces of the self-tuning~\cite{selftune}, self-managing~\cite{selfmanage}, and self-driving~\cite{oracleselfdrive,Pavlocidr17} databases. 


\iffalse

Workload-based optimization, which tunes a database management system (DBMS) to maximize its performance for a specific workload, is a critical aspect of database management and is essential for ensuring that database systems can efficiently handle the demands of modern applications. As a result, a large number of database administrative and performance tuning tools have been developed for workload-based optimization. While workload metrics, such as resource utilization and runtime statistics, may be sufficient for optimizing certain aspects of the system with some of these tools, other workload optimization tools require an understanding of the semantics of queries in the workload, making a workload query trace necessary as input. Physical design tools fall under this category and are provided by many established commercial database products~\cite{sqlserver,db2,oracle,informix}. Prominent examples include Microsoft's AutoAdmin~\cite{autoadmin} and IBM's DB2 design advisor~\cite{db2advisor}. They automatically recommend physical design features, such as indexes, materialized views, partitioning schemes of tables, and multi-dimensional clustering (MDC) of tables~\cite{mdc}, for a given workload of queries. Another related workload-based optimization technique is semantic caching~\cite{DBLP:conf/sigmod/StonebrakerJGP90,DBLP:conf/edbt/ChenR94a,DBLP:conf/vldb/DarFJST96,DBLP:journals/pvldb/DurnerCL21}, which involves caching frequently accessed query results based on the semantic meaning of the queries to accelerate repeated execution. %A third category of workload-based optimization tools automatically recommends the best database configurations for a given workload~\cite{ituned,qtune,ottertune}, such as the buffer pool size, optimizer knobs, memory and disk settings, and degree of parallelism. 
In fact, many of the aforementioned workload-based optimization techniques form the foundational pieces of the self-tuning~\cite{selftune}, self-managing~\cite{selfmanage}, and self-driving~\cite{oracleselfdrive,Pavlocidr17} databases. 
%\yuanyuan{I have removed examples of auto-scaling, as I don't think it is a good example application.}
\fi

\begin{figure}[t!]
   \centering
   \includegraphics[width=0.95\linewidth]{figure/sibyl.pdf}
   \caption{ \sys\ improves workload-based optimization by providing accurately forecasted future query workloads.
   %, compared to using historical queries as input.
   %\yuanyuan{@Hanxian, can you add three dots between view selection and query result caching, to indicate that there are other applications that \sys can support. Also, I think color red is usually used for alarming things. Maybe we change the color red to color blue or green?}
   }
   \label{fig:sibyl}
      \vspace{-15pt}
 \end{figure}


For workload-based optimization, the input workload plays a crucial role and needs to be a good representation of the expected workload. 
Traditionally, historical query traces have been used as input workloads  with the assumption that workloads are mostly \emph{static}. However, as we discuss in \S\ref{sec:motivation}, real workloads exhibit highly recurring query structures with changing patterns in both their arrival intervals and data accesses.
For instance, query templates are often shared across users, teams, and applications, but may be customized with different parameter values to access varying data at different points in time. Consider a log analysis query that reports errors for different devices and error types: \texttt{"SELECT * FROM T WHERE device = ? AND errorType = ? AND eventDate BETWEEN ? AND ?"}. Although the query template is recurring, the parameter values may be customized depending on the reporting needs, e.g., different devices may be analyzed on different days of the week, and the granularity of the time interval may switch from daily to weekly over weekends. Thus, optimization recommendations (\eg recommended views) based solely on historical queries may not be effective for such time-evolving workload patterns. Instead, by accurately predicting the changes in patterns, optimization tools can tune over a more representative workload, resulting in improved performance and resource utilization.




 %To achieve the optimization goal in these workload-based optimization techniques, the input workload of queries plays a crucial role. It needs to be a good representation of the expected workload. Historical query traces have typically been used as input workloads for these tools, with the assumption that workloads do not change much. However, as we will demonstrate in \S\ref{sec:motivation}, our observation on various production workloads reveals that although queries in real workloads are highly recurrent (sharing similar query logics or query templates), most of them exhibit time-evolving behavior (the parameter values of queries with the same template change over time). As a result, optimizations or recommendations based solely on historical queries may not be effective for future workloads. Example 1 below demonstrates a scenario where materialized view recommendation based on historical query trace cannot benefit future queries in a time-evolving workload. This example can also be generalized to other scenarios of workload-based optimization. 

%\textsc{Example 1}: In a workload that frequently queries and analyzes the last 7-day's data, the query trace for Jan 25, 2023 contains a frequently occurring subexpression \texttt{"SELECT * FROM T WHERE event\_date BETWEEN `01/18/2023' AND `01/25/2023'"}. If this query trace is used as the input workload to recommend materialized views for the next day, it will likely materialize this common computation. However, on Jan 26, 2023, this recommended view will be useless since the frequently occurring subexpression will become \texttt{"SELECT * FROM T WHERE event\_date BETWEEN `01/19/2023' AND `01/26/2023'"}. 

%A wide range of existing database administrative tools assume that workloads are static, including popular physical design tools provided by commercial database products such as Microsoft's AutoAdmin~\cite{autoadmin} and IBM's DB2 design advisor~\cite{db2advisor}~\cite{sqlserver,db2,oracle,informix}. These tools automatically recommend physical design features like indexes, materialized views, partitioning schemes, and multi-dimensional clustering (MDC) of tables, based on a workload of queries as input, while considering system constraints like storage budgets. Typically, historical query traces have been used as input workloads for these tools. However, since real workloads exhibit time-evolving behavior, recommendations based solely on historical data may not be effective for future workloads. For example, recommended views based on queries with old predicate parameter values may not be useful for future queries if the predicate parameters change over time.



\iffalse
To adapt to evolving workloads, these workload-based optimization tools can be modified and enhanced to accommodate workload changes, e.g. by incorporating predicting capabilities, or alternatively, applied \textit{without modification} by substituting the history workload with a workload that accurately represents the anticipated query trace in the future. This motivates the need for forecasting future workload.
\fi

%Another area that can benefit from workload forecasting is semantic caching~\cite{DBLP:conf/sigmod/StonebrakerJGP90,DBLP:conf/edbt/ChenR94a,DBLP:conf/vldb/DarFJST96,DBLP:journals/pvldb/DurnerCL21}, which involves caching query results based on their definitions to accelerate repeated executions. Forecasting the workload can help populate the semantic cache proactively by executing queries before users submit them, thereby improving performance.

%Lastly, auto-scaling, which involves automatically adjusting system resources such as compute power and storage based on usage, is another important category of database administrative tasks, especially in the cloud. Many existing auto-scaling approaches are reactive, making resource allocation decisions based on immediate historical usage. By substituting historical usage with the expected usage of forecasted workloads, these reactive auto-scaling tools can be directly applied for proactive auto-scaling~\cite{das16, Delimitrou14, Floratou17}.\hanxian{remove auto-scaling?}



As depicted in Table~\ref{tab:comparison}, prior research works~\cite{ma2018query,meduri2021evaluation,abebe2022tiresias} have made efforts to forecast different aspects of future workload, but none have addressed the challenge of predicting  future query traces with both precise \textit{query statements} and their anticipated \textit{arrival time} for \textit{time-evolving} workloads. The approach proposed by Meduri et al.~\cite{meduri2021evaluation} takes the current query as input and predicts the next query by forecasting query fragments separately and then assembling them into a complete query statement. However, predicting fragments individually can result in invalid queries, requiring identification and repair of errors. For predicting the literals (or parameters) used in the query statement, \cite{meduri2021evaluation} only forecasts a bin of possible values instead of the exact values. Furthermore, this approach only considers the current query as input, neglecting the time-evolving characteristics of the workload from a time-series perspective. QueryBot 5000~\cite{ma2018query} and Tiresias~\cite{abebe2022tiresias} focus on forecasting the \textit{arrival rate} of future query workload by training on patterns from historical query arrival rates. %So, with QueryBot\_5000, 
As a result, 
%one can predict, in a coarser grain, what types of queries and how many of them are expected in the future. 
these techniques can only predict the types of queries and the number of them expected in the future in a coarse granularity.
Yet they %cannot 
do not generate %provide 
the specific query statements for those workload-based optimization tools that require understanding the semantics of queries, especially in the context of time-evolving workloads.
%like in Example~1.
%QueryBot\_5000 leverages ensemble learning~\cite{opitz1999popular} to average the results of linear regression and RNNs. The linear regression does not support incremental fine-tuning and necessitates retraining from scratch for workload shifts. 
%We summarize the comparison between \sys\ and these two most related works in Table~\ref{tab:comparison}. 

To address these limitations, we propose \sys, an end-to-end machine learning (ML)-based workload forecasting framework, which can accurately predict \emph{both} the future query statements and their arrival time as well as automatically capture the varying recurring patterns across multiple evolving templates in a workload. The forecasted workloads can be then used to help improve the workload-based optimization as shown in Figure~\ref{fig:sibyl}.
%\sys also automatically captures the varying recurring patterns across multiple evolving templates in a workload
%Table~\ref{tab:comparison} compares \sys\ with the three aforementioned  closely related works.
We next highlight the major contributions of \sys.
%Other previous studies~\cite{holze2008autonomic,holze2010towards} only forecast the shifts of the workload. Query2Vec~\cite{jain2018query2vec} learns the vector representation for query plans to perform workload summarization and query classification. %It focuses on capturing the syntax similarity among queries but fails to predict the literals in queries.


%For instance, Meduri et al.~\cite{meduri2021evaluation} takes the current query and recommend the next query fragments by predicting fragments separately then reconstructing them into a query statement. However, forecasting fragments separately easily results in ill-formed or invalid queries and requires additional SQL violation fixing. For the literal forecasting, they forecast a bin of constants in the future query rather than the exact values, which is not precise. Thus, they suggest an approximate future query rather than an exact future query. Moreover, this paper only looks at the current query as input while overlooking the time-evolving characteristics in a sequence perspective. QueryBot\_5000~\cite{ma2018query} predicts the arrival rate of future query workload by learning on the historical arrival rate patterns. It leverages ensemble learning~\cite{opitz1999popular} to average the results of linear regression and RNNs. The linear regression does not support incremental fine-tuning and requires to train from scratch for workload shifts. We summarize the comparison among \sys\ and these two most related works in Table~\ref{tab:comparison}. Other previous work~\cite{holze2008autonomic,holze2010towards} only forecast the shifts of the workload. Query2Vec~\cite{jain2018query2vec} learns the vector representation for query plans to perform workload summarization and query classification. It focuses on capturing the syntax similarity among queries but fails to predict the literals in queries. None of the previous works is able to address the challenging task of precisely predicting future query workloads.

\Huge
\begin{table}[t!]
  \caption{ \sys\ vs. three closely related works.
  %\tar{do we mean templates by query statements? Otherwise they will have literals too.}\hanxian{I think template has no literals, while query statement has?} \tar{ then predicting statements captures literals too? how can [37] predict statements but not literals.}\hanxian{the emphasis is on "specific". [37] predicts statement with a blur range of literals -- \ie first make all possible numbers of the literal into 10 bins, then predict which bin.} \tar{double check the changes below. let's be a bit careful while choosing words to avoid confusion}
  }
  
  %\hanxian{TODO: add and double check Khuzaima et al.}%\rana{increase font} 
  %\tar{we could also add a row for capturing drifts (or fine-tuning) which prior works dont capture.}%\tar{double check that CMU paper doesn't capture views}\hanxian{CMU paper did not capture views, only index}
  %\sys\ Comparison among \sys\ and the two most related works. %\tar{This table is nice, maybe we should discuss if we want to move this to intro/motivation.}\hanxian{It was in the intro; but it takes a very long paragraph to explain each $\checkmark$ and $\times$}}
  %\tar{the last three rows are basically saying the same thing? Can we replace them with a single row saying Forecast Precise SQL Statements and for Meduri et al we can put a dash or ? saying partial.}
 % }
  \label{tab:comparison}

  
\resizebox{0.95\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{lccc}
\hline
& \begin{tabular}[c]{@{}c@{}}QueryBot 5000~\cite{ma2018query}\\  Tiresias~\cite{abebe2022tiresias}\end{tabular}
    & Meduri et al.~\cite{meduri2021evaluation}  & \sys\    \\ \hline
What to predict     & Query arrival rate & Next query         & \begin{tabular}[c]{@{}c@{}}Future queries\\ \& arrival time\end{tabular} \\ \hline
Methods & \begin{tabular}[c]{@{}c@{}}Hybrid-ensemble \\Learning\end{tabular} & \begin{tabular}[c]{@{}c@{}}RNNs \&\\ Q-learning\end{tabular} & \sysModel\ \\ \hline
Applications       & \multicolumn{1}{c}{Index selection}    & \begin{tabular}[c]{@{}c@{}}Query\\ recommendation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Physical design tools,\\ semantic caching \end{tabular}     \\ \hline
\begin{tabular}[l]{@{}l@{}}Time-evolving \\forecasting\end{tabular} %\tar{rename this to Future Arrival Rates?}
&    \textcolor{green!70!black}{\checkmark}     &   \textcolor{red}{$\times$}    &     \textcolor{green!70!black}{\checkmark} \\ \hline
\begin{tabular}[l]{@{}l@{}}%Various \tar{Variable?} 
Variable prediction \\windows\end{tabular}   &    \textcolor{green!70!black}{\checkmark}     &   \textcolor{red}{ $\times$}    &     \textcolor{green!70!black}{\checkmark} \\ \hline
%\begin{tabular}[l]{@{}l@{}}Forecast the exact\\ future queries\end{tabular}     &   \textcolor{red}{$\times$}    &  \textcolor{red}{$\times$}    &    \textcolor{green!70!black}{\checkmark}     \\ \hline
\begin{tabular}[l]{@{}l@{}}Forecast future\\ query statement  \end{tabular}       &   \textcolor{red}{$\times$}    &  \begin{tabular}[c]{@{}c@{}}\textcolor{green!70!black}{\checkmark}\tnote{$\ddag$} \end{tabular}
&    \textcolor{green!70!black}{\checkmark}     \\ \hline
%\begin{tabular}[l]{@{}l@{}}Well-formed\\ query statement\end{tabular}       &   \textcolor{red}{$\times$}    &  \textcolor{red}{$\times$}    &    \textcolor{green!70!black}{\checkmark}     \\ \hline
\begin{tabular}[l]{@{}l@{}}Forecast \emph{precise}\\ query parameter values\end{tabular}       &   \textcolor{red}{$\times$}    &  \textcolor{red}{$\times$}\tnote{$\ddag$}   &    \textcolor{green!70!black}{\checkmark}     \\ \hline
%\begin{tabular}[l]{@{}l@{}}Efficient workload\\ representation\end{tabular}     &    \textcolor{green!70!black}{\checkmark}   &  \textcolor{red}{$\times$}    &    \textcolor{green!70!black}{\checkmark}     \\ \hline
%\begin{tabular}[l]{@{}l@{}}Incremental fine-\\tuning on drifts\end{tabular}      &   \textcolor{red}{$\times$}    &    \textcolor{green!70!black}{\checkmark}&     \textcolor{green!70!black}{ \checkmark} \\ \hline
\end{tabular}

 \begin{tablenotes}
    %\footnotesize
    \huge
    \item[$\ddag$] Meduri et al.~\cite{meduri2021evaluation} forecast future query statement with coarse-grained parameter value ranges.
  \end{tablenotes}

\end{threeparttable}
 
 
 }
\vspace{-15pt}
\end{table}

\normalsize


\vspace{-2mm}
\subsection{\sys\ Contributions}

%In this paper, we introduce \sys, an end-to-end machine learning-based workload forecasting framework. Our framework aims to achieve the challenging goal of accurately predicting \emph{both} the future query statements as well as their arrival time. Furthermore,  a workload may have multiple evolving templates with varying recurring patterns which aim to automately capture in our framework.

%Our goal in 
%The goal of this work is to accurately predict \emph{both} the future query statements and their arrival time. To achieve this goal, we present \sys, an end-to-end machine learning-based workload forecasting framework. \sys also automatically captures the varying recurring patterns across multiple evolving templates in a workload.

%a workload may have multiple evolving templates with varying recurring patterns which aim to automately capture in our framework.

%By addressing this broader but also more challenging workload forecasting problem, our aim is to enable a wide range of existing workload-based optimization tools that were originally designed for static workloads to be directly applied \textit{without modification} for time-evolving workloads. 

%The myriad benefits of a holistic future workload forecasting technique for improving applications in DBMS are evident as illustrated above. This entails forecasting the entire query statements as well as the query arrival time for a sequence of queries within a defined time span. The forecasting horizon, determined by the interval for performing optimization techniques in DBMS, plays a crucial role. For instance, being able to predict all future queries that will arrive within the next view selection interval would enable the view selection algorithm to proactively adapt to the evolving workload and optimize performance.

% All these benefits call for a holistic future workload forecasting technique, to improve applications in DBMS. %as shown in Figure~\ref{fig:sibyl}. 
% To explore such forecasting, we identify the exact future query workloads forecasting problem, \ie forecasting the entire query statements precisely as well as the query arrival time for the future query sequence in a time span. The time span is the forecasting horizon decided by the interval to perform the optimization techniques in DBMS. \Eg it is ideal that we can predict all future queries that will be arriving in the next view selection interval to help the view selection algorithm be aware of the workload evolution and improve the performance.




\begin{comment}
Our aim is to \textit{accurately capture the evolving nature of workloads over time and forecast the precise future query workloads across different horizons, in order to enhance various applications in DMBS}. To accomplish this, we first conduct a comprehensive study on four real workloads: %Windows Telemetry (WT)~\cite{wtcituscon},
\mssales,\wmc, %SCOPE~\cite{chaiken2008scope}, 
\scope, 
%MSSales 
and BusTracker~\cite{ma2018query}. We present three crucial observations: (1) workloads are evolving over time rather than static. It is crucial to capture the time-evolving nature of the workload by learning through the past queries in the history; (2) A large portion (over $94.5\%$ in our study) of the workload queries repeat frequently with only the constants in the filter predicates changed, \aka query templates are recurring. It is wise to reuse the recurring query templates in future workload forecasting. (3) We further study the predictability of query parameters which motivate us to develop an accurate forecasting framework. We show the details of the study in \S\ref{sec:motivation}.
\end{comment}

%Meanwhile, we present two crucial observations that motivate us to propose our categorization and forecasting framework. According to our study on three real workloads (Windows Mission Control~\cite{} (WMC), SCOPE~\cite{}, BusTracker~\cite{ma2018query}), we observe that: (1) workloads are evolving over time, especially the value of parameters \hanxian{"parameter" or "attribute"? "parameter value" or "constant"? need to be unified in the whole paper} in the filter predicates. (2) A large portion (more than $93.3\%$) of the workload queries repeats frequently with only the filter parameters changed, \aka query templates (query with constants in the predicates removed) are re-occurring periodically. Especially, the daily templates are the majority in the workload as shown in Figure~\ref{fig:RecurringTemplates}. This gives us the opportunity to reuse the periodically recurring query templates. 

%Based on the aforementioned observations, we propose \sys, a holistic framework that effectively characterizes and forecasts evolving workloads to improve DBMS workload-dependent optimization techniques. %\sys\ utilizes a template-based representation to encode query statements and arrival time as a feature map, which is used for training and testing ML models. \sys\ employs a novel encoder-decoder ML model, \sysModel, to learn and predict future query templates, constants in the templates, and query arrival time. Additionally, \sys\ introduces a \cutNpack\ technique to cluster templates and train one ML model for each cluster, optimizing model capacity, prediction time, and storage efficiency. %The key contributions of \sys\ are summarized as follows:

%We qualitatively and quantitatively study on four real workloads and draw insights in terms of their re-occurrence, evolving patterns, and predictability, which motivates the design of \sys.
    %We conduct qualitative and quantitative studies on four real workloads, gaining insights into their re-occurrence, evolving nature, and predictability, which motivate the design of \sys.
We motivate the \sys design %based on 
by qualitative and quantitative studies on four real workloads (\S\ref{sec:motivation}). We identify three %crucial 
insights from our observations: 1) real workloads are highly recurrent (sharing the same \textit{query templates} but with different \textit{query parameters}) as discussed earlier; 2) these recurrent queries often exhibit time-evolving behavior; and 3) they are highly predictable. Based on these insights, we first formalize a %simple 
next-$k$ workload forecasting problem that predicts the next $k$ queries in the future for each query template. We develop an ML-based technique %\sys\ 
that seamlessly integrates both query arrival time and query parameters into a common framework, and forecasts the \emph{entire} statements of future recurrent queries and their arrival time. %Specifically,
To this end, we develop a template-based featurization method that captures a large number of parametric 
expressions (\S\ref{sec:featureEngineer}), and combine stacked LSTM~\cite{hochreiter1997long} with an encoder-decoder architecture~\cite{cho2014learning}, resulting in a model that we refer to as \sysModel (\S\ref{sec:templatemodels}), to better capture both the temporal dependencies and the possible inter-dependencies among query parameters, for \textit{per-template}, multi-variate, multi-step, time-series prediction.


We further identify a set of practical challenges in order to make the predictions usable for performance tuning tools. 
%However, there are some practical challenges that we need to address to make the predictions usable within performance tuning tools.
%For example, 
First, it is difficult to pre-determine the right number of queries ($k$) to forecast, to produce a useful workload for database optimization tools. Rather, a more practical version of the problem is to forecast the future queries for the next time interval $\Delta t$. But the number of queries expected in next $\Delta t$ varies substantially across templates.
%The template size (i.e., the expected number of queries for the template in next $\Delta t$ time interval) typically vary in real workloads. %Furthermore, 
Second, with one model per template, we need to limit the number of models to ensure the scalability of our design. To address these two issues, we extend the solution for the next-$k$ problem to the next-$\Delta t$ forecasting problem (\S\ref{sec:design-delta}). For templates with large expected numbers of queries, we `cut' them into sub-templates in order to employ the predicted next-$k$ queries to produce results for the next-$\Delta t$ problem. To reduce the number of models, we %also 
`pack' templates with a small expected number of queries into bins. We then build per-bin models (\S\ref{sec:perbinmodel}). %This
Our approach not only %provides 
yields accurate results for the next-$\Delta t$ forecasting problem, but also reduces the number of \sysModel\ models by up to $23\times$, resulting in a significant reduction in both time and storage overhead by up to $13.6\times$ and $6\times$, respectively. 

%Another 
A third practical challenge is that real-world workloads change dynamically, i.e., new templates may emerge, while old templates may become less relevant. The evolving patterns of literals may also change. To capture such changes, %within our framework, 
\sys\ %provides 
adopts a feedback loop to handle workload shifts
(\S\ref{sec:feedbackloop}). %It
The feedback loop uses incremental learning to adapt the pre-trained \sysModel\ to the shifted workloads, achieving accuracy comparable to full training, with only a few seconds of fine-tuning overhead.

%Overall, 
We integrate the forecasting model with the feedback loop to develop the end-to-end forecasting solution of \sys. The paper also discusses customizable effectiveness measurement for specific use cases, and presents a common effectiveness measurement that can be utilized for many performance tuning tools (\S\ref{sec:accuracy}).
We evaluate \sys\ on four real workloads (\S\ref{sec:eval}) and demonstrate its accurate forecasting ability. Furthermore, we apply \sys\ to two database applications on real workloads: materialized view selection and semantic caching of query results. Our results show $1.7\times$ improvement in view selection and $8.6\times$ improvement in semantic caching using forecasted workloads compared to historical workloads. %highlighting the efficacy of \sys.

%\textbf{Outline}. The rest of this paper is organized as follows:    \S\ref{sec:motivation} elaborates our study on real workloads and shows our motivation. \S\ref{sec:Problem} defines the query forecasting problem and \S\ref{sec:overview} gives an overview of \sys. \S\ref{sec:design-k} and \S\ref{sec:design-delta} detail the solutions for the next-$k$ forecasting and the next-$\Delta t$ forecasting problem. The online feedback loop is described in \S\ref{sec:feedbackloop}. We discuss customizable effectiveness measurement in \S\ref{sec:accuracy}. \S\ref{sec:eval} presents our evaluation followed by \S\ref{sec:related} where we review the related work. Finally, we conclude in \S\ref{sec:conclusion}.  
%\vspace{-2mm}
%\tar{double check the outline}

%,~\ref{sec:scalable} ~\ref{sec:opt}. 
%We show two selected applications in  \S\ref{sec:apps}, which are used in further evaluations and discussions in  \S\ref{sec:eval}.
%We present our evaluation in \S\ref{sec:eval}, discuss on related work in  \S\ref{sec:related} and conclude the paper in \S\ref{sec:conclusion}.

    
    %\item %To reuse the highly-recurrent templates, \sys\ deploys a template-based featurization. It wisely simplifies the forecasting problem compared to token-based featurization~\cite{jain2018query2vec,meduri2021evaluation} and generates well-formed query statements. It is more efficient and takes $13.8\times$ smaller feature maps storage overhead compared to bit-vector representation~\cite{meduri2021evaluation}.
  %  We propose a ML-based framework \sys\ to solve both versions of the query forecasting problem, consisting of (1) a tailored template-based featurization to reuse recurrent templates and better represent the time-evolving features. (2) \sysModel, an adapted encoder-decoder neural network for time-series learning and multi-query prediction problem, achieving an average $F1$ score of $86.9\%$.
    %employs a template-based featurization to reuse highly-recurrent templates, simplifying the forecasting problem compared to token-based featurization methods. It generates well-formed query statements and is more efficient, with $13.8 \times$ smaller storage overhead compared to token-basesd representation.

    %\item %We adapt the encoder-decoder architecture and propose \sysModel\ for time-series learning and multi-query prediction problem with an average accuracy of \todox{$xxx\%$}. We improve the framework scalability and reduce the number of \sysModel\ models to train for each workload with a template \cutNpack\ method and significantly improve time and storage efficiency by up to \todox{$xxx\times$}.
    
    %To solve the variable template trace length problem in real workloads, we propose a template \cutNpack\ approach to reorganize templates and reduce the number of \sysModel\ models by up to $23\times$, resulting in significant reduction on time and storage overhead by up to $13.6\times$ and $6.0\times$. 

    %\item %\sys\ provides a feedback loop to deal with workload shift and a mechanism to handle new emerging templates. Specifically, \sys\ leverages incremental learning to efficiently adapt the pre-trained \sysModel\ onto the shifted workloads, with \todox{$xxx\%$} accuracy improvement and \todox{$xxx\times$} less training time compared to re-train the models from scratch.

    %\sys\ provides a feedback loop to handle workload shifts and new emerging templates. It leverages incremental learning to efficiently adapt the pre-trained \sysModel\ onto shifted workloads, achieving almost the same accuracy as a full training process, with only a few seconds fine-tuning overhead.


    %\item  %We demonstrate the usefulness of \sys\ with two real applications: view selection and query results caching on  \mssales\ and \wmc\ real workloads, respectively and show up to 45\% improvement on \mssales\ and \todox{} on \wmc\ compared to the ones without foresting. \sys\ is valuable to improve the DBMS performance in multiple aspects and achieve autonomous DBMS.
    %We showcase the efficacy of \sys\ through two real-world applications: view selection and query results caching on \mssales\ and \wmc\ workloads, respectively. Our results reveal up to $6.5\times$ improvement on \mssales\ and $7.6\times$ on BusTracker compared to approaches without forecasting. %\sys\ is a valuable tool for enhancing DBMS performance in various aspects and enabling autonomous DBMS operations.
%\squishend


%\sys\ first categorizes the parameters according to their predictability. Then \sys\ deploys a template-based representation to encode the whole query text as a feature vector, upon which ML models can be trained and tested. \sys\ learns and predicts evolving workloads by novel encoder-decoder ML models. Furthermore, \sys\ improves the prediction time and storage efficiency by clustering the templates. In each cluster, we learn one ML model to forecast the whole query text in the future consisting of templates and all the constants in the templates. We evaluate \sys\ on two applications: view materialization and indexing, on four real workloads (Windows Mission Control, SCOPE, BusTracker, MSSales) and show \todox{$xxx\%$} and \todox{$xxx\%$} improvement accordingly. We summarize our contributions as follows: \hanxian{emphasize our tech novelty}
%\begin{itemize}
%    \item We propose \sys\, a general query-based workload forecasting framework, which is valuable to improve the DBMS performance in multiple aspects and achieve autonomous DBMS.
%    \item We characterize and categorize four real workloads and draw insights in terms of the re-occurrence, evolution, and predictability for the evolving workloads.
%    \item We propose a novel encoder-decoder neural network to learn over the past workloads and forecast the future workloads as well as their arrival time preciously and efficiently, enhanced with the novel clustering method.
%    \item Experiments show effectiveness and improvement on view materialization and index selection compared to other state-of-the-art models. 
%\end{itemize}

%To the best of our knowledge, \sys\ is the first framework to identify and solve the future queries forecasting problem for time-evolving workload. \sys\ learns and forecasts the entire statements of future recurrent queries in various time spans with their corresponding arrival time. \tar{To the best of our knowledge, \sys\ is the first framework that learns and forecasts the \emph{entire} statements of future recurrent queries in various time spans with their corresponding arrival time.}

%\noindent\textbf{Outline}. The rest of this paper is organized as follows:    \S\ref{sec:motivation} elaborates our study on real workloads and shows our motivation.  \S\ref{sec:Problem} defines the query forecasting problem and \S\ref{sec:overview} gives an overview of \sys. \S\ref{sec:design-k} and \S\ref{sec:design-delta} detail the solutions for the next-$k$ queries forecasting and the next-$\Delta t$ forecasting problem. We offer applicable customization in \S\ref{sec:customization}. %,~\ref{sec:scalable} and~\ref{sec:opt}. 
%We show two selected applications in  \S\ref{sec:apps}, which are used in further evaluations and discussions in  \S\ref{sec:eval}.
%We present our evaluation in \S\ref{sec:eval}, discuss on related work in  \S\ref{sec:related} and conclude the paper in \S\ref{sec:conclusion}.




==> backup_content/3-problem.backup.tex <==
% \begin{figure}[t!]
% \centering
% \begin{sqllisting}
% (*@\textbf{Query Q}@*):
% SELECT A.x, A.y, SUM(A.e) / SUM(A.z) AS val
% FROM A
% WHERE A.val1 = 'v1' AND A.val2 = 'v2' AND A.val3 IN (1,2)
% GROUP BY A.x, A.y

% (*@\textbf{\textit{Template temp(Q)}}@*):
% SELECT A.x,A.y, SUM(A.e) / SUM(A.z) AS val
% FROM A
% WHERE A.val1 = $1 AND A.val2 = $2 AND A.val3 IN $3
% GROUP BY A.x, A.y

% (*@\textbf{\textit{Parameters para(Q)}}@*):
% ('v1', 'v2', (1,2))
% \end{sqllisting}

% \caption{Templatization Example\hanxian{Since we removed the `parameterized query' in \S3, shall we remove this figure or move it to \S5.1?} \rana{Moved to \S5.1}}
% \label{lst:template}
% \vspace{-15pt}
% \end{figure}
%\section{Preliminaries and Overview} \label{sec:Problem}
\vspace{-2mm}
\section{Problem Statement}
\label{sec:Problem} %rana{lock}


% \yuanyuan{Maybe the following paragraph can be moved to intro. But for now I will put it here.} \rana{I agree -- moved to the intro}

% The rationale behind focusing on this broader workload forecasting problem is to allow a wide range of existing database administrative tools that were originally optimized for static workloads to be used directly \textit{without modification} for time-evolving workloads. A prominent example category of such tools is physical design tools, which are provided by many established commercial database products~\cite{sqlserver,db2,oracle,informix}. These tools, with notable examples such as Microsoft's AutoAdmin~\cite{autoadmin} and IBM's DB2 design advisor~\cite{db2advisor}, automatically recommend physical design features, such as indexes, materialized views, partitioning schemes of tables, and multi-dimensional clustering (MDC) of tables~\cite{mdc}. They all take in a workload of queries W as input and generate recommendations for a selected set of features, by minimizing the total cost of W, while adhering to system constraints, such as storage budgets. Traditionally, historical traces of queries have been used as input workloads for these tools. However, as real workloads exhibit time-evolving behavior, recommendations based on historical data may not work well for future workloads. For instance, recommended views based on queries with old predicate parameter values may not be useful for future queries if the predicate parameters change over time. To adapt to evolving workloads, these tools can be modified to include predicting capabilities or alternatively, applied without modification by substituting the history workloads with the forecasted workloads as input. Another related area that can benefit from forecasting is semantic caching~\cite{DBLP:conf/sigmod/StonebrakerJGP90,DBLP:conf/edbt/ChenR94a,DBLP:conf/vldb/DarFJST96,DBLP:journals/pvldb/DurnerCL21}, which involves caching query results based on their definitions to accelerate repeated executions. Forecasting the workload can help to populate the semantic cache eagerly by executing queries before users submit them, thereby improving performance. 
% %\yuanyuan{I will consider adding the semantic data caching application here too. }\jesus{I added some contents}
% Lastly, another important category of database administrative tasks, especially on cloud, is auto scaling, i.e. automatically adjusting the resources allocated to the system (\eg compute power and storage) based on usage. Many existing auto-scaling approaches are \textit{reactive}~\cite{das16, Delimitrou14, Floratou17}, deciding on resource allocation based on immediate historical usage. By substituting historical usage with the expected usage of forecasted workload, these reactive auto-scaling tools can be directly applied without a change for \textit{proactive} auto scaling.

%\subsection{Problem Formulation}

We begin by introducing  key concepts to  %that help us 
formally define the workload forecasting problem. 
% Before formulating the formal definition of the workload forecasting problem that we are solving, we first start with the definition of some basic concepts.
% We refer a \textit{query} $q$ as a statement written in SQL or a similar language, such as the \scope query language. It should be noted that the definition of a query in this paper is broad and encompasses insert, delete, or update statements as well, although the four workloads we study in this paper primarily contain query statements only.
A \textit{query}, denoted by $q$, refers to a statement expressed in SQL or a similar language, such as \scope query language. %It is worth noting that our definition of a query is broad, encompassing not only \texttt{SELECT} statements, but also \texttt{INSERT}, \texttt{DELETE}, or \texttt{UPDATE} statements. However, this work primarily focuses on workloads that predominantly consist of \texttt{SELECT} statements. 
% \textit{Parameterized query} is a type of query that utilizes \textit{parameters} to enhance both its flexibility and security. It separates the query logic from the parameters, with the query logic referred to as the \textit{query template}. Within the query template, placeholders are included for the parameters. For a normally written query, we can rewrite it into a parameterized query by extracting the constant values used in the query as parameters. For a query $q$, we denote $temp(q)$ as the template of $q$, and $para(q)$ as the sequence of parameter values of $q$. For example, the query \texttt{"SELECT * FROM event WHERE event\_time >=`Jan 22, 2023' AND event\_time <=`Jan 29, 2023'"} can be rewritten as a parameterized query with \texttt{"SELECT * FROM event WHERE event\_time >=\$1 AND event\_time <\$2"} as the template, and \texttt{(`Jan 22, 2023', `Jan 29, 2023')} as the parameter values.
%A \textit{parameterized query} is a query type that enhances flexibility and security by utilizing \textit{parameters}. It separates the query logic into a \textit{query template}, which contains placeholders for the parameters. The constant values used in a regular query can be extracted as parameters to convert it into a parameterized query. For a query denoted as $q$, we define $temp(q)$ as the template of $q$, and $para(q)$ as the sequence of parameter values used in $q$. Figure~\ref{lst:template} shows a templatization  example. 
%\tar{maybe we should add a line or two to explain whether we perform any normalization for templates that may look different (e.g., different ordering of parameters) but are same.}\hanxian{@Jesus, in \S5.1, AST equivalent checking, did we distinguish different parameter order?}\jesus{Is the definition of parameterized query needed for our problem definition though? It seems it is part of the solution rather than the problem (and as such, we already describe it in 5.1)}
A \textit{workload}, denoted by $W$, is defined as a time series of queries, where each query $q_i$ in the workload has an associated arrival time $t_{q_i}$ indicating when the query is issued.  Queries in the workload are ordered based on their arrival time, i.e., $t_{q_1} \leq t_{q_2} \leq ... \leq t_{q_n}$. Hence, the workload can be represented as $W=[(q_1, t_{q_1}), (q_2, t_{q_2}), ..., (q_n, t_{q_n})]$.

In this work, we present the formal definitions of two workload forecasting problems: next-$k$ forecasting and next-$\Delta t$ forecasting.

\begin{definition} (Next-$k$ Forecasting) \\ Given a workload $W=[(q_1, t_{q_1}), (q_2, t_{q_2}), ..., (q_n, t_{q_n})]$, the next-$k$ forecasting problem predicts the next $k$ future queries as:
$$F_k(W) = [(q_{n+1}, t_{q_{n+1}}), (q_{n+2}, t_{q_{n+2}}), ..., (q_{n+k}, t_{q_{n+k}})]$$
\end{definition}

\begin{definition} (Next-$\Delta t$ Forecasting) \\ Given a workload $W=[(q_1, t_{q_1}), (q_2, t_{q_2}), ..., (q_n, t_{q_n})]$, the next-$\Delta t$ forecasting problem predicts the queries in the next time interval of size $\Delta t$ as:
$$F_{\Delta t}(W) = [(q_{n+1}, t_{q_{n+1}}), (q_{n+2}, t_{q_{n+2}}), ..., (q_{n+\sigma}, t_{q_{n+\sigma}})]$$ where $t_{q_{n+\sigma}}<t_{q_{n}}+\Delta t \leq t_{q_{n+\sigma+1}}$  .
\end{definition}

In contrast to the fixed number of queries to predict in next-$k$ forecasting, the next-$\Delta t$ forecasting deals with the prediction of queries within a fixed time interval. 
In real-world applications, determining the target time interval of the expected future queries is often more feasible than the target number of future queries. 
For instance, database tuning tasks are typically performed at regular intervals, such as hourly, daily, or weekly. Thus, having knowledge of the expected workload in the target time interval is crucial for optimizing database performance and resource utilization. 
%We define the next-$\Delta t$ forecasting problem as follows:

The next-$\Delta t$ forecasting problem is more challenging than the next-$k$ forecasting problem as the number of queries to predict, $\sigma$, is not known in advance and must be determined based on the arrival time of the predicted queries. 
Operationally, the forecasting model needs to keep predicting queries until it sees a query with an arrival time exceeding the next $\Delta t$ time interval.  
The anticipated arrival time of each query is an essential component of the forecasting task as it determines the ordering of the predicted queries and constrains the forecast for the next-$\Delta t$ prediction challenge. 

%Note that while prior work have focused on predicting either the next coming query~\cite{meduri2021evaluation} or arrival rates of queries~\cite{ma2018query} in future workloads, \sys\ focuses specifically on the task of forecasting \textit{a time series of queries} that will appear in the future workload. 
%In the rest of the paper, we first give an overview of \sys~(\S\ref{sec:overview}) followed by describing our solution to the simpler next-$k$ forecasting problem~(\S\ref{sec:design-k}). We then extend the next-$k$ forecasting  solution to tackle the more complex next-$\Delta t$ forecasting problem~(\S\ref{sec:design-delta}). 


%It is important to recognize that the anticipated arrival time of each query is an essential component of the forecasting task. The arrival time not only determines the ordering of the predicted queries, but it also constrains the forecast for the next-$\Delta t$ prediction challenge. %In certain database applications, such as auto-scaling, having knowledge of the expected query arrival time is critical for optimal allocation of resources. \tar{we may want to remove the last line if we don't evaluate on auto-scaling?}

%The problem of next-$k$ forecasting is relatively simple, as the number of queries to predict is fixed. However, in the next-$\Delta t$ forecasting problem, the number of queries to predict is not known in advance and must be determined based on the arrival time of the predicted queries: operationally we have to keep predicting queries until we see a query with arrival time exceeding the next $\Delta t$ time interval. This makes the prediction task more challenging, but at the same time the next-$\Delta t$ forecasting problem is often more practical for real-world applications. Database administrative tasks, such as selecting materialized views and adjusting the allocated resources on cloud, are typically performed at regular intervals, such as hourly, daily, or weekly. Therefore, having the knowledge of the expected workload in the target time interval is essential for optimizing database performance and resource utilization. It is more often the case that based on the target database administrative task, we can determine the target time interval of the expected future queries (next-$\Delta t$) rather than the target number of future queries (next-$k$). Ultimately, \sys is designed to solve the more challenging next-$\Delta t$ forecasting problem. In this paper, we start with solving the simpler next-$k$ forecasting problem, then extend our solution to tackle the next-$\Delta t$ forecasting problem.

%\tar{we may want to briefly hint here that the evaluation metric for the above problems is dependent or needs to customized for each application and we cover in Section x.}\hanxian{Metrics are the same. The only difference is that whether we know the length of forecasting.}

\begin{comment}

Our goal is to forecast the exact future workload, \ie the entire statement of future queries in a time span, with the corresponding query arrival time. We now define some basic concepts and the \textit{exact future workload forecasting problem} formally.

%\yuanyuan{Should we introduce two versions of the problem? The ultimate probelm we want to solve is to forecast a sequence of queries with arrival time for a given time interval. A simpler version of the problem is to predict a sequence of n future queries with arrival time. Section 5 is to tackle the simpler problem first, then section 6 solves the ultimate problem.}

\textsc{Definition 1.} [Query] A query is the query statement requesting information from a database written in a query language, \eg SQL. We represent a query as $q_t$ with query arrival time $t$.

\textsc{Example 2.} An example of a query statement: 
\colorbox{gray!20}{SELECT * FROM}
\colorbox{gray!20}{event WHERE event\_time >=Jan 22 AND event\_time <=Jan 29}


\textsc{Definition 2.} [Template] A template is the query statement with constants in the filter predicates excluded. Based on our observations (See Section~\ref{sec:evolvingPatterns}) that parameters in the filter predicates are evolving, we mainly focus on them and exclude them in the templates while leaving other constants not in filter predicates in the templates. Each template is assigned a unique query template ID \textit{qtid} in a workload.

\textsc{Example 3.} The template for the query in Example 2: 
\colorbox{gray!20}{SELECT *}
\colorbox{gray!20}{FROM event WHERE event\_time >= \$1 AND event\_time <= \$2}. 


\textsc{Definition 3.} [Workload] A workload is a collection of query traces in the order of query arrival time $q_{t_1}, q_{t_2}, ..., q_{t_{|W|}}$, where $|W|$ is the length of query traces.

\textsc{Definition 4.} [Evolving Workload] Evolving workload consists of queries with parameters changing over time.

\textsc{Definition 5.} [Exact Future Workload Forecasting] Given a sequence of past queries $q_1, q_2, ..., q_n$ and their arrival time $t_{q_{1}}$, $t_{q_{2}} ...t_{q_{n}}$ from a workload until the current time step, the exact future workload forecasting is to predict the future query sequence $q_{n+1}, q_{n+2}, ... , q_{n+m}$ and their corresponding arrival timestamps $t_{q_{n+1}}$, $t_{q_{n+2}}, ...,t_{q_{n+m}}$. $n$ denotes the past sequence length and $m$ denotes the future sequence length, which are customized by applications. Formally, the exact future workload forecasting is a function $\mathcal{F}$:
\begin{equation}\label{eq:forecasting}
\small
    \mathcal{F}(q_1, q_2, ..., q_n;t_{q_{1}}, t_{q_{2}}, ...,t_{q_{n}}) = q_{n+1}, q_{n+2}, ... , q_{n+m};t_{q_{n+1}},t_{q_{n+2}},...,t_{q_{n+m}}
\end{equation}

Based on the above observation that the templates are highly recurrent and the filter parameters show common evolving patterns (see Section \ref{sec:motivation}), \sys\ deploys template-based preprocessing and featurization. Thus, \sys\ forecasts a query by forecasting its template and all the excluded parameter values in the template:
\begin{equation}
q_i \ = \ <qtid_{q_i}, param_1, param_2,...param_{|P|_{qtid_{q_i}}}>
\end{equation}
where $|P|_{qtid_{q_i}}$ is the total number of parameters in template $qtid_{q_i}$. We then fill the corresponding predicted parameters into the templates to
be the future queries. %Previous work QueryBot\_5000~\cite{ma2018query} only forecasts the query arrival rate; by forecasting the future query arrival time $t_{q_{n+1}},t_{q_{n+2}},...,t_{q_{n+m}}$, \sys\ is able to derive the number of queries in a certain time window. Meduri et al. ~\cite{meduri2021evaluation} only forecast the next query $q_{n+1}$, without the arrival time. Query2Vec~\cite{jain2018query2vec} learns only the representation of query template, without parameters or arrival time. \sys\ aims to forecast the precious workload.

We now discuss two versions of the exact future workload forecasting:

\textsc{Definition 6.} [Next k-queries forecasting] Specifically, the forecasting sequence length is $k$. Given the observation that parameters in a template are evolving, for each template, we propose to train one model to forecast all the parameters in the future next $k$ queries with arrival time in Section~\ref{sec:design}. We refer it as the \textit{per-template} model.

\textsc{Definition 7.} [Next time-interval forecasting] Specifically, the forecasting sequence length is the number of all the queries in the next time interval, and the time interval is specified by the application. Since various templates have various number of queries, \aka volume, in a certain observation time interval, \sys\ then applies a \cutNpack\ algorithm to slice the large volume templates and group small volume templates to fit into the model forecasting window size, \aka bin. We then propose the \textit{per-bin} model to forecast the next time-interval queries for each bin in Section~\ref{sec:scalable}.

\hanxian{Per-bin Model: cut and pack algorithm fits templates into equal-size bin. Need a better name here. "per-group" / "per-cluster"?? Template re-group / re-cluster?}

\tar{
%A few things are missing. 
%1) Define evolving, templates, etc. 
%2) What we think reoccurs vs what can change (i.e., unseen) in the past? 
%3) We perhaps need to also tell our focus is on filter/predicate forecasting? 
4) Briefly tell how the output will be used by application such view materialization or index tuning.}\rana{TODO}


\subsection{Evaluation Metrics}\label{sec:goals}
The goal of \sys\ is to predict future queries accurately and the forecasted queries help improve the applications in DBMS.

\noindent\textbf{Forecasting accuracy}
A main goal of \sys\ is to predict future queries accurately. 

\textsc{Definition 8.} [Forecasting Accuracy] Given the forecasted queries $\hat{q}_{n+1}, \hat{q}_{n+2}, ... , \hat{q}_{n+m}$ and the ground truth $q_{n+1}, q_{n+2}, ... , q_{n+m}$, the forecasting accuracy is defined as $Acc = \frac{|\hat{q}_{n+i}=q_{n+i}|}{m}, \forall i \in [1,m]$.

%Thus we prefer the predicted query sequence $\hat{q}_{n+1}, \hat{q}_{n+2}, ... , \hat{q}_{n+m}$ that is exactly the same as the ground truth future query $q_{n+1}, q_{n+2}, ... , q_{n+m}$, \ie $ \hat{q}_{n+i}=q_{n+i}, \forall i \in [1,m] $. 


\noindent\textbf{Time and storage efficiency}
Whe also consider the time and storage overhead when providing an accurate future workload forecasting. The time overhead consists of the time of: (1) offline stage: workloads preprocessing and ML models training; (2) online stage: workload forecasting and periodically model fine-tuning. The storage overhead consists of the memory consumption to store the feature maps that represent the workload and to store all the pre-trained models. As the increasing complexity of today's workloads, how to achieve high accuracy with low time and storage overhead, to provide a scalable forecast framework is challenge and is our goal.

\end{comment}

\begin{comment}
\subsection{Challenges} 
There are three main challenges in building a forecasting framework for real-world workloads. \hanxian{I may rephrase or remove this subsection later, because the challenges are mentioned when introducing the detailed techniques.} \tar{Yes, we need to compress this subsection.}

\noindent\textbf{Support general workloads representation} The first challenge is to represent the workload in a general method so that: (1) the machine learning model is allowed to take the past queries and forecast the future queries based on the representation. Moreover, how to represent the workload decides how the feature map is encoded. A good query representation catches the key features that are critical and necessary in the model training. (2) the representation is general and can be reused in most common DBMS types. Based on the above observation that the templates are highly recurring and the filter parameters show common evolving patterns, \sys\ breaks down the problem by templatizing the queries and encoding the predicates. To be more preciously, we first identify the recurring templates (queries without filter parameter values) in the workload. Then for a given a high frequent template $Temp1$, there are $s$ attributes in the filter predicates $p^1, p^2, ... , p^s$. For each of the parameter $p^k$, we learn from the past sequence of it $p^k_1, p^k_2, ..., p^k_n$ and predict the future window of it $p^k_{n+1}, p^k_{n+2},..., p^k_{n+m}$. Then we fill the corresponding predicted parameters into the templates to be the future queries.

\noindent\textbf{Support diverse patterns learning} The second challenge is how to capture different patterns and workload features perfectly. Not only do different workloads have different patterns, but a single workload can also have patterns with various shapes or periods combined. Thus, an effective forecasting model must be able to identify and characterize patterns that are occurring simultaneously within the same workload. To solve the second challenge, \sys\ first characterizes and categorizes the workloads, then proposes a novel LSTM-based encoder-decoder neural network that can learn different types and different periods of patterns for all the parameters at the same time.

\noindent\textbf{Support large query volumes} The third challenge is that applications execute millions of queries per day (shown in Table~\ref{tab:3statistics}). Thus, we have a huge amount of training data collected from daily queries. Moreover, the models are required to be updated periodically since the workload patterns can be dynamic and change over time. How to support efficient model training and model updating is critical in practice for real-world workloads. Previous paper~\cite{ma2018query} aims to predict query arrival rate, and it performs downsampling and heavily reduces the dataset volume by \todox{$?? \times$} by only counting the number of queries in one minute. However, in our problem, we aim to predict the exact query text in the whole sequence. Any downsampling will skew the time-evolving patterns and change the data distribution. Another large-volume issue is the prediction volume problem. Since our target application is view selecting, which is performed at a daily frequency. It is required that our models can predict one day volume's future queries at a time. This corresponds to $\sim 10,000 / 43,000 / 44,000$ queries per day for WT / SCOPE / BusTracker. It is difficult to build such a forecasting model to predict such a large volume at a time. To solve this challenge, \sys\ first proposes to train one model to predict for one template, and later proposes to cluster various workloads based on the workload features and adjust the pre-template model to the pre-cluster model to improve model efficiency.

\end{comment}

==> backup_content/7-optimization.backup.tex <==

%\section{Customization} \label{sec:opt}
%\tar{are the below optimizations not needed by other applications such as index tuning?}\hanxian{7.1 and 7.2 can be customized according to any application (\ie how the application is going to use the forecasted workload). 7.3 is more general}
%\yuanyuan{I think any application is likely to use some customization here, not just for MV. In addition I don't think Section 7.3 is for customization. Feedback loop is part of the general ML framework. Maybe we should move 7.3 to Section 5/6, or as a separate section.}

%The training target and definition of a helpful forecasting can be customized by applications. Here we show optimization examples tailored for view selection application.  

\vspace{-2mm}
\section{Effectiveness Measurement}
\label{sec:accuracy}

Measuring the accuracy of the forecasting results highly depends on the specific use case or the application for which we want to forecast the workload. Below we discuss a general metric that can be customized for specific scenarios. Given the predicted workload $\hat{W}$ and the ground-truth future workload $W$, we use recall, precision, and F1 score as our evaluation metric with a customizable function 
$match(W, \hat{W})$ that defines the bag of ground-truth queries in $W$ that are matched by the queries in $\hat{W}$ , and can be tailored to a specific application (details later). More formally, 

{
\small
\begin{equation}\label{eq:recall}
    Recall = \frac{|match(W, \hat{W})|}{|W|}
\end{equation}

\begin{equation}\label{eq:precision}
    Precision = \frac{|match(W, \hat{W})|}{|\hat{W}|}
\end{equation}

\begin{equation}\label{eq:f1}
    F1 = \frac{2 \cdot precision \cdot recall}{precision+recall}
\end{equation}
}

%In the above equations, $match(Q, \hat{Q})$ denotes a correct forecasting identifier function returns $1$ if the forecasted query contains the groundtruth otherwise returns $0$. 
%When checking the \textit{match} function (i.e. multiset, allowing duplicates) of ground-truth queries that are matched to the predicted queries, and can be tailored to a specific application (details later).

%\iffalse
%A derived metric $F1$ score is the harmonic mean of these two metrics:
%\begin{equation}\label{eq:f1}
%    F1 = \frac{2 \cdot precision \cdot recall}{precision+recall}
%\end{equation}

%A high recall represents a high coverage of the ground truth. A high precision shows that the model returns more relevant results than irrelevant ones. 
%A higher $F1$ shows a higher prediction accuracy considering both recall and precision. In this paper, we use all three metrics to measure the accuracy of \sysModel models, while using various definitions of the prediction match function $match(Q, \hat{Q})$.
%\fi

While one can use a strict matching where both parameter values as well as arrival time of forecasted queries exactly matches with the ground truth queries, such a matching is rarely needed. For a large number of applications, such as caching, index tuning, view recommendation, partitioning of tables, and determination of the MDC of tables, a forecasted workload for a specific period of time should cover most of the ground-truth queries. The precise ordering of queries or actual arrival time is insignificant in a targeting time window, rather 
we want to only determine which queries should be included in given time window for which we perform tuning. Thus, the forecasted workload, in the given time window, can be treated as a bag of queries. Similarly, a \textit{containment} metric as described below can be used for matching a ground-truth query with a predicted query.

A query $q_1$ is \textit{contained} in another query $q_2$, i.e., $q_1\subseteq q_2$, if for every database instance $d$, $q_1(d)\subseteq q_2(d)$, where $q_i(d)$ is the bag of tuples resulted in evaluating $q_i$ on $d$. In \sys, we measure containment only using predicate values. For equality predicate, the model gives a single value, hence we perform exact matching. For range predicates, a match is considered if the predicted range contains the ground-truth range. In the case of an IN clause, a match is considered if the predicted value is a superset of the ground-truth value. Given the forecasted query bag $\hat{Q}$ and the ground-truth query bag $Q$, we define the containment-based match as $match_{bag,\subseteq}(W, \hat{W})=\{q\in W \mathrel{|}\exists \hat{q}\in \hat{W}, \mathrel{} q\subseteq \hat{q}\}$. 

To better understand the effectiveness of forecasting in terms of containment, we also want to measure the degree of the containment relationship for each \textit{matched} ground-truth and predicted query pair. We develop a new metric called \textit{average containment-diff ratio} computed as follows. For a predicted range $\hat{R}$ and a ground-truth range $R$, the \textit{containment-diff ratio} is defined as $\frac{|\hat{R}-R|}{|R|}$, where $-$ is the range difference operation. In cases of a half-bounded range predicate, such as $col>a$, all the observed parameter values related to $col$ are used to obtain the upper bound $max_{col}$ and lower bound $min_{col}$, and the range $(a, \infty)$ is changed to $(a, max_{col})$ before computing the containment-diff ratio. Similarly, for IN-clause predicates, given a predicted set $\hat{S}$ and ground-truth set $S$, the containment-diff ratio is defined as $\frac{|\hat{S}-S|}{|S|}$, where $-$ is the set difference operation. A good containment-based match should have a containment-diff ratio close to zero. Finally, the average containment-diff ratio is computed across all range predicates and IN-clause predicates for all the \textit{matched queries} (we do not compute containment-diff ratio for unmatched queries). In \S\ref{sec:eval}, % our empirical evaluation, 
we report the results on both containment-based accuracy as well as average containment-diff ratio.

%To penalize cases where the predicted range predicates or IN-clause predicates overshoot in containment, such as when the predicted range is very large but the ground-truth range is small, we also measure the \textit{average proportional difference} on all the matched queries. Specifically,


\iffalse

\section{Customization}\label{sec:customization}

In this section, we delve into some components \tar{dont see components in this section only accuracy metrics and handling unpredictable parameters?} of \sys that can be tailored to meet the specific needs of the intended application. Additionally, we offer some widely applicable customization options.

\hanxian{As a workload forecasting framework to help improve DBMS optimization tools, \sys\ offers some widely applicable customization options. Here we give an example customization tailored to physical design type of application and semantic caching.}

\subsection{Customized Accuracy Measurement} \label{sec:customized_accuracy}

Measuring the accuracy of the forecasting results highly depends on the specific use case or the application for which we want to forecast the workload. \tar{give a few concrete examples of application and what metrics they need?}\hanxian{@Yuanyuan}

%In some cases, accuracy may be defined as the degree to which the forecasted queries match the actual queries over a specific time period. In other cases, accuracy may be defined based on action that will be taken based on the forecast, such as optimizing performance and resource utilization. 
%As a result, the definition of accuracy is customizable in \sys to fit the specific requirements of the target application.

%\subsection{Forecasting Accuracy}
\subsubsection{\textbf{Metrics}}
Two widely-used accuracy metrics are recall and precision calculating with the predicted workload $\hat{Q}$ and the ground-truth future workload $Q$:



\begin{equation}\label{eq:recall}
    Recall = \frac{|match(Q, \hat{Q})|}{|Q|}
\end{equation}

\begin{equation}\label{eq:precision}
    Precision = \frac{|match(Q, \hat{Q})|}{|\hat{Q}|}
\end{equation}

In the above equations, $match(Q, \hat{Q})$ denotes the bag (i.e. multiset, allowing duplicates) of ground-truth queries that are matched to the predicted queries, and can be tailored to a specific application (details later).


A derived metric $F1$ score is the harmonic mean of these two metrics:
\begin{equation}\label{eq:f1}
    F1 = \frac{2 \cdot precision \cdot recall}{precision+recall}
\end{equation}

A high recall represents a high coverage of the ground truth. A high precision shows that the model returns more relevant results than irrelevant ones. 
A higher $F1$ shows a higher prediction accuracy considering both recall and precision. In this paper, we use all three metrics to measure the accuracy of \sysModel models, while using various definitions of the prediction match function $match(Q, \hat{Q})$.

\subsubsection{\textbf{Prediction Match}}

Various applications have different ways to define how the predicted workload matches with the ground truth. 

\textbf{Strict Match.} \hanxian{A general matching definition in ML field} A straightforward and \textit{strict} matching definition for the next-$k$ forecasting problem is as follows: Given the forecasted query sequence $\hat{Q}=(\hat{q}_{n+1}, \hat{q}_{n+2}, ... , \hat{q}_{n+k})$ and the ground truth $Q=(q_{n+1}, q_{n+2}, ... , q_{n+k})$, we define the bag of strictly matched queries as $match_{\equiv}(Q, \hat{Q})=\{q_{n+i} \in Q \mathrel{|} q_{n+i}= \hat{q}_{n+i}, \mathrel{} \forall i \in [1,k]\}$. And $q_{n+i}=\hat{q}_{n+i}$ is defined as the forecasted feature vector for $q_{n+i}$ is element-wise equal to the ground truth feature vector $\hat{fv}_{n+i}^j=fv_{n+i}^j, \forall j \in |\hat{fv}_{n+i}|$. This definition requires not only the predicted queries match exactly with the ground truth queries, but also the orders of the queries have to match exactly. \tar{maybe give an example of application that needs strict matching?}

%In practical terms, this strict match definition is not particularly relevant or beneficial. Typically, applications are more concerned with the expected queries during a specific time interval in the future, regardless of their order or actual arrival time. Essentially, the predicted query arrival time is only useful in determining which queries should be included in the anticipated workload. By disregarding the order, we can treat the workload in a given time window as a bag of queries.


%\subsubsection{Bag-Oriented Match.} By disregarding the order, we can treat the workload in a given time window as a bag of queries and establish a new match definition.

%Given the forecasted query bag $\hat{Q}$ and the ground-truth query bag $Q$, we define the bag-oriented match as $match_{bag,=}(Q, \hat{Q})=\{q\in Q\mathrel{|} \exists \hat{q}\in \hat{Q},\mathrel{} q= \hat{q}\}$. 


\textbf{Containment-Based Match.}\label{sec:containmentAccuracy}
In practical terms, the above strict match definition is not particularly relevant or beneficial. \tar{if not relevant/beneficial at all, why discuss it?}
For large number of applications, such as caching, index tuning, view recommendation, partitioning of tables, and determination of the MDC of tables, a good forecasted workload for a specific period of time should cover most of the ground-truth queries. First of all, the order of queries or actual arrival time is insignificant. Essentially, the predicted query arrival time is only useful in determining which queries should be included in the anticipated workload. By disregarding the order, we can treat the workload in a given time window as a bag of queries. Secondly, the predicted queries also do not need to exactly match ground-truth queries. We find that often the containment metric is adequate to be considered as a match. 


%Typically, applications are more concerned with the expected queries during a specific time interval in the future, regardless of their order or actual arrival time. Essentially, the predicted query arrival time is only useful in determining which queries should be included in the anticipated workload. By disregarding the order, we can treat the workload in a given time window as a bag of queries.

%For large number of applications, such as caching, index tuning, view recommendation, partitioning of tables, and determination of the MDC of tables, a good forecasted future workload for a specific period of time should cover most of the ground-truth queries. Not only the order of queries is insignificant, the predicted queries also do not need to exactly match ground-truth queries. Often the containment semantic is adequate to be considered as a match. 

In general, a query $q_1$ is \textit{contained} in another query $q_2$, denoted as $q_1\subseteq q_2$, if for every database instance $d$, $q_1(d)\subseteq q_2(d)$, where $q_i(d)$ is the multi-set of the tuples resulted in evaluating $q_i$ on $d$. \hanxian{to answer the below question, we can easily know from the definition of `contained', the mismatch or `some are contained+some are not' are both wrong forecasting; they do not contain ground truth.}

The containment cases that appear in the predicates are only considered. In cases of an equality predicate, the forecasting model always predicts one value for the parameter that must match exactly with the ground truth, disallowing any general containment. For range predicates, a match is considered if the predicted range contains the ground-truth range. In the case of a predicate with an IN clause, a match is considered if the predicted value is a superset of the ground-truth value.

Given the forecasted query bag $\hat{Q}$ and the ground-truth query bag $Q$, we define the containment-based match as $match_{bag,\subseteq}(Q, \hat{Q})=\{q\in Q \mathrel{|}\exists \hat{q}\in \hat{Q}, \mathrel{} q\subseteq \hat{q}\}$. 

To penalize cases where the predicted range predicates or IN-clause predicates overshoot in containment, such as when the predicted range is very large but the ground-truth range is small, we also measure the \textit{average proportional difference} on all the matched queries. Specifically, for a predicted range $\hat{R}$ and a ground-truth range $R$, the proportional difference is defined as $\frac{|\hat{R}|-|R|}{|R|}$. In cases of a half-bounded range predicate, such as $col>a$, all the observed parameter values related to $col$ are used to obtain the upper bound $max_{col}$ and lower bound $min_{col}$, and the range $(a, \infty)$ is changed to $(a, max_{col})$ before computing the proportional difference. Similarly, for IN-clause predicates, given a predicted set $\hat{S}$ and ground-truth set $S$, the proportional difference is defined as $\frac{|\hat{S}|-|S|}{|S|}$. Finally, the average proportional difference is computed across all range predicates and IN-clause predicates for all the matched queries.

\tar{clarify what happens when some parameters mismatch within a query, especially when some are contained and others are not.?}
\fi 

%\hanxian{I commented out the Time-Sensitive Match since we are not using it.}
%\textbf{Time-Sensitive Match.} 
%Query arrival time is very hard to predict precisely at fine granularity, \eg seconds or milliseconds. Even for applications in which the query arrival time does matter, it is not necessary to have precise accuracy at such a granular level. In such cases, we can break the prediction time window into smaller windows (\eg hourly windows for $\Delta t=1 day$), and compute the accuracy metrics for each small window using either the multi-set-oriented or containment-based match definition, and then use the average accuracy across windows as the final accuracy. \tar{how does this interplay with cut and pack algorithm?}


%\noindent\textbf{General Definition:} A main goal of \sys\ is to predict future queries accurately. Given the forecasted queries $\hat{q}_{n+1}, \hat{q}_{n+2}, ... , \hat{q}_{n+m}$ and the ground truth $q_{n+1}, q_{n+2}, ... , q_{n+m}$, a general forecasting accuracy is defined as $Acc = \frac{|\hat{q}_{n+i}=q_{n+i}|}{m}, \forall i \in [1,m]$. And $\hat{q}_{n+i}=q_{n+i}$ is defined as the forecasted feature vector for $q_{n+i}$ is element-wise equal to the ground truth feature vector $\hat{fv}_{n+i}^j=fv_{n+i}^j, \forall j \in |\hat{fv}_{n+i}|$.

%Thus we prefer the predicted query sequence $\hat{q}_{n+1}, \hat{q}_{n+2}, ... , \hat{q}_{n+m}$ that is exactly the same as the ground truth future query $q_{n+1}, q_{n+2}, ... , q_{n+m}$, \ie $ \hat{q}_{n+i}=q_{n+i}, \forall i \in [1,m] $. 
\begin{comment}
\noindent\textbf{Optimized Definition:} Considering the final goal of \sys\ is to improve optimization techniques in DBMS with the forecasted workload, the definition of a correct forecasting is adjustable according to the applications to serve. Taking view selection as an example, if the views based on the forecasted workload can answer the future query workload, we consider it as a correct forecasting. \Eg if the forecasted query statement is the same as the ground truth, only with some forecasted parameter values in the filter the supersets of the ground truth values, it is treated as a useful and correct forecasting. However, if the forecasted query is partially correct with wrong query statement or wrong constants, the view cannot answer the ground truth future query, which is considered as a wrong prediction. An example is shown to illustrate the customized correctness.

\textsc{Example 4.} The correct and wrong forecasting customized by view selection application \\
The ground truth query: \colorbox{gray!20}{SELECT * FROM table WHERE 3<t<7}\\
A correct forecasting: \colorbox{gray!20}{SELECT * FROM table WHERE 3<t<7}\\
A correct forecasting: \colorbox{gray!20}{SELECT * FROM table WHERE \textbf{2<t<8}}\\
A wrong forecasting: \colorbox{gray!20}{SELECT * FROM table WHERE \textbf{5<t<8}} \\
%A wrong forecasting: \colorbox{gray!20}{SELECT * FROM \textbf{event} WHERE 3<t<7} \\

%Besides considering the containment, we also remove the unpredictable parameters in the feature vector and rewrite the queries to \textit{groupby} the unpredictable parameters. In this way, we ensure the view materialized based on the forecasted feature vectors with only the highly predictable parameters can cover the ground truth. 
Moreover, we do not emphasis whether the order of queries in the forecasted sequence is exactly the same as the ground truth sequence in a certain time interval. In real workload, the queries can be committed in a high frequency, \eg every milliseconds in WT. It is unlikely to forecast the arrival miiliseconds precisely. And It is not necessary to forecast the query order correctly in a finer grain than the observation time interval. Since the forecasted sequence will help applications in the format of a batch of queries in a time interval, instead of a sequence of queries. But we still show the majority of the sequence is in a relatively correct order with high accuracy for various $\Delta t$ settings in \S\ref{sec:eval}.
\end{comment}

\begin{comment}
\subsection{Customized Training Object}
We design the learning object customized by the exact forecasting problem. As mentioned in \S\ref{sec:motivation}, the majority of predictable parameters follows the time-evolving patterns while there can be some outliers. Therefore, we deploy Huber Loss~\cite{huber1992robust}, which is a robust loss function and is less sensitive to outliers in data than the na\"ive mean square error or mean absolute error. Since the target is exact query forecasting, it is required that the forecasting for all elements, \ie template ID and parameters, in the feature vectors are correct. We define the loss of model training as the mean of all the individual forecasting on every single element in the feature vectors to encourage the models to learn forecasting individually and simultaneously correct. Given the ground truth feature map $f=[{fv}_1,{fv}_2,...,{fv}_t]$ over time span $t$, with each feature vector $fv_i=[fv_i^1, fv_i^2,...,fv_i^s] $ consisting $s$ parameters to forecast, and given a prediction on the feature map $\hat{f} = [\hat{fv}_1,\hat{fv}_2,...,\hat{fv}_t]$, the loss function is define as:

\begin{align}
\mathcal{L}oss(f, \hat{f}) &= \sum_{i=1}^t\sum_{k=1}^s \mathcal{L}oss (fv_i^k, \hat{fv}_i^k)\\
\text{Where} \ \ \mathcal{L}oss (fv_i^k, \hat{fv}_i^k)&=\begin{cases}
  \frac{1}{2}(fv_i^k-\hat{fv}_i^k)^2, & \text{for} \ \ |fv_i^k-\hat{fv}_i^k|\leq \delta \\
  \delta(|fv_i^k-\hat{fv}_i^k|-\frac{1}{2}\delta), & \text{otherwise}
\end{cases}
\end{align}
\end{comment}


%\label{sec:unpredicatable}
\textbf{Handling unpredictable parameters.} Since we give entire query statements as part of the workload to the tuning applications, we need to provide values for unpredictable parameters (even though the percentage of such parameters is small as discussed in \S\ref{sec:motivation}). While handling such parameters depends on the applications, we propose the following approach that can be used for many tuning applications, including the ones we consider in this work. Specifically, we generalize the corresponding predicate into a catch-all predicate, \textit{TRUE}. As an example, for the template \texttt{"SELECT ... FROM ... WHERE id = \$1 AND age > \$2 ..."}, if parameter \$1 is unpredictable, we transform its predicate \texttt{"id = \$1"} to \texttt{"TRUE"}, with predicted query as \texttt{"SELECT ... FROM ... WHERE TRUE AND age > 18 ..."}. By this generalization, we ensure that a forecasted query with accurate values for all the predictable parameters is a containment-based match to the ground truth.
%\vspace{-2mm}

%\tar{maybe remind how you identify unpredictable parameters?}
\iffalse
For a large number of physical design related applications, where the containment semantics is most appropriate for defining a prediction match, an unpredictable parameter in a predicate can be handled by generalizing the corresponding predicate into a catch-all predicate, \textit{TRUE}. As an example, for the template \texttt{"SELECT ... FROM ... WHERE id = \$1 AND age > \$2 ..."}, if parameter \$1 is unpredictable, we can transform its predicate \texttt{"id = \$1"} to \texttt{"TRUE"}, then a predicted example query will look like \texttt{"SELECT ... FROM ... WHERE TRUE AND age > 18 ..."}. By this generalization, we can make sure that a forecasted query with accurate values for all the predictable parameters is a containment-based match to the ground truth.
\fi

==> content/1-intro.backup.tex <==
\section{Introduction}
%\yuanyuan{@Hanxian, please go over all figures to make sure that the workload names have been changed to the ones we are currently using. e.g. Figure 9 is still using the old names for sigmod submission.}
\begin{comment}
Optimization techniques in DBMSs such as view selection~\cite{mami2012survey,zhou2006dynamic}, query results caching~\cite{DBLP:conf/vldb/DarFJST96}, index recommendation~\cite{gani2016survey, das2019automatically}, partitioning~\cite{agrawal2004integrating,curino2010schism}, \etc usually assume workloads are static. With the rapid development of today's data-driven applications and the growing complexity of big data, conventional techniques with the static workload assumption are sub-optimal. We demonstrate the importance of workload forecasting with view selection as a motivation application:

%\jcr{I think we could elaborate a bit more in the following example by using a few (couple) filter conditions, each one with different characteristics, to showcase that it is not as simple as assuming that everything is a sliding time window}
\textsc{Example 1.} A workload recurrently queries the last week's data and a high frequent query's filter on Jan 25th is
\colorbox{gray!20}{WHERE event\_date}\\ \colorbox{gray!20}{>= Jan 18th  AND event\_date <= Jan 25th}. The values of predicates `event\_date >=' and `event\_date <=' in the WHERE clause are changing upon query arrival time. They are `Jan 18th' AND `Jan 25th' on Jan 25th's queries while changing to `event\_date >= Jan 19th AND event\_date <= Jan 26th' in Jan 26th's queries, etc. 

The conventional view selection techniques (\eg~\cite{zhou2006dynamic}) assume workloads are static and select views based on statistics of the historical queries, \eg the high frequent historical query with filter predicates `event\_date >= Jan 22 AND event\_date <= Jan 29'. The materialized views based on the historical predicate values cannot answer the future query since the real values are changing over query time, which leads to a sub-optimal solution. 
%view selection example is shown in Figure~\ref{fig:moti}: conventional view recommendation ~\cite{zhou2006dynamic} assumes the workload is static and materializes highly frequent historical queries, but fails to capture the workload evolving features. 
The optimal materialization results are hard to derive by only considering the highly frequent historical queries while ignoring the time-evolving nature of the workloads. This calls for a new forecasting technique that captures the time-evolving characteristics of the workloads in a long-time horizon and forecasts the future workloads precisely. 

% \begin{comment}
% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=\linewidth]{figure/example2.pdf}
%   \caption{Motivation example. Conventional view selection assumes the workload is static and materializes the result of historical query, which fails to answer the future query. With \sys, view selection is performed based on the forecasted workload and improve \todox{$xxx\times$} performance.
%   \hanxian{seems too much texts in the figure? should I separate the example with the SIBYL workflow?}}
%   \label{fig:moti}
% \end{figure}
 \end{comment}


%\jcr{Consider introducing this paragraph (how useful can forecasting be) before talking about the example and the complexity of doing it right.}
\begin{comment}
Moreover, forecasting future query statements as well as their corresponding arrival time before they really arrive benefits DBMS in many aspects. By predicting the future queries that will arrive in the next forecasting interval, DBMS is allowed to speculatively execute the queries and skip the execution when the actual future queries arrive, thereby improving performance. Workload forecasting also helps auto-tuning the DMBS ahead of time: forecasting the possible values of constants in selection (or join) predicates can help DBMS create indexes and views; forecasting the future query as well as the arrival time give valuable hints to perform better auto-scaling; forecasting the set of tables and attributes in predicates allows DBMS to construct partial or full query plan ahead of time; forecasting the sort (ORDER BY) and aggregate (COUNT) operator to help DBMS in pre-allocation of buffer pages and configuring \# CPU-bound threads to parallelize the execution, etc. %\hanxian{Need help here to elaborate the potential benefit of our framework. And why predicting a sequence of queries + arrival time is critical. What \sys\ can do but other works cannot do, e.g., VM?} \textcolor{gray}{COPY-PASTE from TODS'21 paper: If we can predict the next SQL query in its entirety during the user think time, then we can speculatively execute it and prefetch its results into the memory. When the actual next query arrives, we can skip its execution and return the prefetched results directly from the memory. Even if an SQL query cannot be predicted in its entirety, knowing apriori the impending query operators and their associated schema elements (defined as query fragments) from the successive query is useful. If we know the set of tables and attributes participating in projection/selection/join/aggregate predicates, then it can allow for partial or full query plan construction during the user think time. The database can also evaluate it partially or entirely depending on the structure of the SQL query. Predicting sort (ORDER BY) and aggregate (COUNT) operator fragments can help in pre-allocation of buffer pages and configuring \# CPU-bound threads to parallelize their execution. Likewise, being cognizant of the selection (or join) predicates can help us pre-load or create indexes if we know the possible range of constants in the selection predicates.}
\end{comment}

Workload-based optimization, which tunes a database management system (DBMS) to maximize its performance for a specific workload, is a critical aspect of database management and is essential for ensuring that database systems can efficiently handle the demands of modern applications. As a result, a large number of database administrative and performance tuning tools have been developed for workload-based optimization. While workload metrics, such as resource utilization and runtime statistics, may be sufficient for optimizing certain aspects of the system with some of these tools, other workload optimization tools require an understanding of the semantics of queries in the workload, making a workload query trace necessary as input. Physical design tools fall under this category and are provided by many established commercial database products~\cite{sqlserver,db2,oracle,informix}. Prominent examples include Microsoft's AutoAdmin~\cite{autoadmin} and IBM's DB2 design advisor~\cite{db2advisor}. They automatically recommend physical design features, such as indexes, materialized views, partitioning schemes of tables, and multi-dimensional clustering (MDC) of tables~\cite{mdc}, for a given workload of queries. Another related workload-based optimization technique is semantic caching~\cite{DBLP:conf/sigmod/StonebrakerJGP90,DBLP:conf/edbt/ChenR94a,DBLP:conf/vldb/DarFJST96,DBLP:journals/pvldb/DurnerCL21}, which involves caching frequently accessed query results based on the semantic meaning of the queries to accelerate repeated execution. %A third category of workload-based optimization tools automatically recommends the best database configurations for a given workload~\cite{ituned,qtune,ottertune}, such as the buffer pool size, optimizer knobs, memory and disk settings, and degree of parallelism. 
In fact, many of the aforementioned workload-based optimization techniques form the foundational pieces of the self-tuning~\cite{selftune}, self-managing~\cite{selfmanage}, and self-driving~\cite{oracleselfdrive,Pavlocidr17} databases. 
%\yuanyuan{I have removed examples of auto-scaling, as I don't think it is a good example application.}
\begin{figure}[t!]
   \centering
   \includegraphics[width=\linewidth]{figure/sibyl.pdf}
   \caption{\sys\ improves workload-based optimization tools with the forecasted future query workloads.
   %\yuanyuan{@Hanxian, can you add three dots between view selection and query result caching, to indicate that there are other applications that \sys can support. Also, I think color red is usually used for alarming things. Maybe we change the color red to color blue or green?}
   }
   \label{fig:sibyl}
      \vspace{-10pt}
 \end{figure}

 
To achieve the optimization goal in these workload-based optimization techniques, the input workload of queries plays a crucial role. It needs to be a good representation of the expected workload. Historical query traces have typically been used as input workloads for these tools, with the assumption that workloads do not change much. However, as we will demonstrate in \S\ref{sec:motivation}, our observation on various production workloads reveals that although queries in real workloads are highly recurrent (sharing similar query logics or query templates), most of them exhibit time-evolving behavior (the parameter values of queries with the same template change over time). As a result, optimizations or recommendations based solely on historical queries may not be effective for future workloads. Example 1 below demonstrates a scenario where materialized view recommendation based on historical query trace cannot benefit future queries in a time-evolving workload. This example can also be generalized to other scenarios of workload-based optimization. 

\textsc{Example 1}: In a workload that frequently queries and analyzes the last 7-day's data, the query trace for Jan 25, 2023 contains a frequently occurring subexpression \texttt{"SELECT * FROM T WHERE event\_date BETWEEN `01/18/2023' AND `01/25/2023'"}. If this query trace is used as the input workload to recommend materialized views for the next day, it will likely materialize this common computation. However, on Jan 26, 2023, this recommended view will be useless since the frequently occurring subexpression will become \texttt{"SELECT * FROM T WHERE event\_date BETWEEN `01/19/2023' AND `01/26/2023'"}. 

%A wide range of existing database administrative tools assume that workloads are static, including popular physical design tools provided by commercial database products such as Microsoft's AutoAdmin~\cite{autoadmin} and IBM's DB2 design advisor~\cite{db2advisor}~\cite{sqlserver,db2,oracle,informix}. These tools automatically recommend physical design features like indexes, materialized views, partitioning schemes, and multi-dimensional clustering (MDC) of tables, based on a workload of queries as input, while considering system constraints like storage budgets. Typically, historical query traces have been used as input workloads for these tools. However, since real workloads exhibit time-evolving behavior, recommendations based solely on historical data may not be effective for future workloads. For example, recommended views based on queries with old predicate parameter values may not be useful for future queries if the predicate parameters change over time.




To adapt to evolving workloads, these workload-based optimization tools can be modified and enhanced to accommodate workload changes, e.g. by incorporating predicting capabilities, or alternatively, applied \textit{without modification} by substituting the history workload with a workload that accurately represents the anticipated query trace in the future. This motivates the need for forecasting future workload.


%Another area that can benefit from workload forecasting is semantic caching~\cite{DBLP:conf/sigmod/StonebrakerJGP90,DBLP:conf/edbt/ChenR94a,DBLP:conf/vldb/DarFJST96,DBLP:journals/pvldb/DurnerCL21}, which involves caching query results based on their definitions to accelerate repeated executions. Forecasting the workload can help populate the semantic cache proactively by executing queries before users submit them, thereby improving performance.

%Lastly, auto-scaling, which involves automatically adjusting system resources such as compute power and storage based on usage, is another important category of database administrative tasks, especially in the cloud. Many existing auto-scaling approaches are reactive, making resource allocation decisions based on immediate historical usage. By substituting historical usage with the expected usage of forecasted workloads, these reactive auto-scaling tools can be directly applied for proactive auto-scaling~\cite{das16, Delimitrou14, Floratou17}.\hanxian{remove auto-scaling?}

\Huge
\begin{table}[t!]
  \caption{ \sys\ vs. QueryBot\_5000~\cite{ma2018query} and Meduri et al.~\cite{meduri2021evaluation}.%\rana{increase font} 
  %\tar{we could also add a row for capturing drifts (or fine-tuning) which prior works dont capture.}%\tar{double check that CMU paper doesn't capture views}\hanxian{CMU paper did not capture views, only index}
  %\sys\ Comparison among \sys\ and the two most related works. %\tar{This table is nice, maybe we should discuss if we want to move this to intro/motivation.}\hanxian{It was in the intro; but it takes a very long paragraph to explain each $\checkmark$ and $\times$}}
  }
  \label{tab:comparison}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccc}
\hline
& QueryBot\_5000~\cite{ma2018query}    & Meduri et al.~\cite{meduri2021evaluation}  & \sys\    \\ \hline
What to predict     & Query arrival rate & Next query         & \begin{tabular}[c]{@{}c@{}}Future queries\\ \& arrival time\end{tabular} \\ \hline
Methods & \begin{tabular}[c]{@{}c@{}}Ensemble \\Learning\end{tabular} & \begin{tabular}[c]{@{}c@{}}RNNs \&\\ Q-learning\end{tabular} & \sysModel\ \\ \hline
Applications       & \multicolumn{1}{c}{Index selection}    & \begin{tabular}[c]{@{}c@{}}Query\\ recommendation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Physical design tools,\\ semantic caching \end{tabular}     \\ \hline
\begin{tabular}[l]{@{}l@{}}Time-evolving \\characteristics\end{tabular} &    \textcolor{green!70!black}{\checkmark}     &   \textcolor{red}{$\times$}    &     \textcolor{green!70!black}{\checkmark} \\ \hline
\begin{tabular}[l]{@{}l@{}}Various prediction \\windows\end{tabular}   &    \textcolor{green!70!black}{\checkmark}     &   \textcolor{red}{ $\times$}    &     \textcolor{green!70!black}{\checkmark} \\ \hline
%\begin{tabular}[l]{@{}l@{}}Forecast the exact\\ future queries\end{tabular}     &   \textcolor{red}{$\times$}    &  \textcolor{red}{$\times$}    &    \textcolor{green!70!black}{\checkmark}     \\ \hline
\begin{tabular}[l]{@{}l@{}}Forecast future\\ query statement\end{tabular}       &   \textcolor{red}{$\times$}    &  \textcolor{green!70!black}{\checkmark}    &    \textcolor{green!70!black}{\checkmark}     \\ \hline
\begin{tabular}[l]{@{}l@{}}Well-formed\\ query statement\end{tabular}       &   \textcolor{red}{$\times$}    &  \textcolor{red}{$\times$}    &    \textcolor{green!70!black}{\checkmark}     \\ \hline
\begin{tabular}[l]{@{}l@{}}Forecast specific\\ query literals\end{tabular}       &   \textcolor{red}{$\times$}    &  \textcolor{red}{$\times$}   &    \textcolor{green!70!black}{\checkmark}     \\ \hline
%\begin{tabular}[l]{@{}l@{}}Efficient workload\\ representation\end{tabular}     &    \textcolor{green!70!black}{\checkmark}   &  \textcolor{red}{$\times$}    &    \textcolor{green!70!black}{\checkmark}     \\ \hline
%\begin{tabular}[l]{@{}l@{}}Incremental fine-\\tuning on drifts\end{tabular}      &   \textcolor{red}{$\times$}    &    \textcolor{green!70!black}{\checkmark}&     \textcolor{green!70!black}{ \checkmark} \\ \hline
\end{tabular}}
\vspace{-5mm}
\end{table}

\normalsize


Prior research has made efforts to forecast different aspects of future workload, but none have addressed the challenge of predicting the future query trace with both actual \textit{query statements} and their anticipated \textit{arrival time} for \textit{time-evolving} workload. The approach proposed in~\cite{meduri2021evaluation} takes the current query as input and predicts the next query by forecasting query fragments separately and then assembling them into a complete query statement. However, predicting fragments individually can result in ill-formed or invalid queries and require additional SQL violation fixing. For predicting the literals (or parameters) used in the query statement, it only forecasts a bin of possible values rather than the exact value. Furthermore, this approach only considers the current query as input, neglecting the time-evolving characteristics of the workload from a time-series perspective. QueryBot\_5000~\cite{ma2018query} focuses on forecasting the \textit{arrival rate} of future query workload by training on patterns from historical query arrival rates. So, with QueryBot\_5000, one can predict, in a coarser grain, what types of queries and how many of them are expected in the future. It cannot provide the specific query statements for those workload-based optimization tools that requires understanding the semantics of queries, especially in the context of time-evolving workloads, like in Example~1. %QueryBot\_5000 leverages ensemble learning~\cite{opitz1999popular} to average the results of linear regression and RNNs. The linear regression does not support incremental fine-tuning and necessitates retraining from scratch for workload shifts. 
We summarize the comparison between \sys\ and these two most related works in Table~\ref{tab:comparison}. Other previous work~\cite{holze2008autonomic,holze2010towards} only forecast the shifts of the workload. Query2Vec~\cite{jain2018query2vec} learns the vector representation for query plans to perform workload summarization and query classification. %It focuses on capturing the syntax similarity among queries but fails to predict the literals in queries.


%For instance, Meduri et al.~\cite{meduri2021evaluation} takes the current query and recommend the next query fragments by predicting fragments separately then reconstructing them into a query statement. However, forecasting fragments separately easily results in ill-formed or invalid queries and requires additional SQL violation fixing. For the literal forecasting, they forecast a bin of constants in the future query rather than the exact values, which is not precise. Thus, they suggest an approximate future query rather than an exact future query. Moreover, this paper only looks at the current query as input while overlooking the time-evolving characteristics in a sequence perspective. QueryBot\_5000~\cite{ma2018query} predicts the arrival rate of future query workload by learning on the historical arrival rate patterns. It leverages ensemble learning~\cite{opitz1999popular} to average the results of linear regression and RNNs. The linear regression does not support incremental fine-tuning and requires to train from scratch for workload shifts. We summarize the comparison among \sys\ and these two most related works in Table~\ref{tab:comparison}. Other previous work~\cite{holze2008autonomic,holze2010towards} only forecast the shifts of the workload. Query2Vec~\cite{jain2018query2vec} learns the vector representation for query plans to perform workload summarization and query classification. It focuses on capturing the syntax similarity among queries but fails to predict the literals in queries. None of the previous works is able to address the challenging task of precisely predicting future query workloads.

In this paper, we introduce \sys, an ML-based workload forecast framework for predicting a time series of future query statements with their arrival time in various prediction windows for time-evolving workloads. By addressing this broader but also more challenging workload forecasting problem, our aim is to enable a wide range of existing workload-based optimization tools that were originally designed for static workloads to be directly applied \textit{without modification} for time-evolving workloads.

%The myriad benefits of a holistic future workload forecasting technique for improving applications in DBMS are evident as illustrated above. This entails forecasting the entire query statements as well as the query arrival time for a sequence of queries within a defined time span. The forecasting horizon, determined by the interval for performing optimization techniques in DBMS, plays a crucial role. For instance, being able to predict all future queries that will arrive within the next view selection interval would enable the view selection algorithm to proactively adapt to the evolving workload and optimize performance.

% All these benefits call for a holistic future workload forecasting technique, to improve applications in DBMS. %as shown in Figure~\ref{fig:sibyl}. 
% To explore such forecasting, we identify the exact future query workloads forecasting problem, \ie forecasting the entire query statements precisely as well as the query arrival time for the future query sequence in a time span. The time span is the forecasting horizon decided by the interval to perform the optimization techniques in DBMS. \Eg it is ideal that we can predict all future queries that will be arriving in the next view selection interval to help the view selection algorithm be aware of the workload evolution and improve the performance.




\begin{comment}
Our aim is to \textit{accurately capture the evolving nature of workloads over time and forecast the precise future query workloads across different horizons, in order to enhance various applications in DMBS}. To accomplish this, we first conduct a comprehensive study on four real workloads: %Windows Telemetry (WT)~\cite{wtcituscon},
\mssales,\wmc, %SCOPE~\cite{chaiken2008scope}, 
\scope, 
%MSSales 
and BusTracker~\cite{ma2018query}. We present three crucial observations: (1) workloads are evolving over time rather than static. It is crucial to capture the time-evolving nature of the workload by learning through the past queries in the history; (2) A large portion (over $94.5\%$ in our study) of the workload queries repeat frequently with only the constants in the filter predicates changed, \aka query templates are recurring. It is wise to reuse the recurring query templates in future workload forecasting. (3) We further study the predictability of query parameters which motivate us to develop an accurate forecasting framework. We show the details of the study in \S\ref{sec:motivation}.
\end{comment}

%Meanwhile, we present two crucial observations that motivate us to propose our categorization and forecasting framework. According to our study on three real workloads (Windows Mission Control~\cite{} (WMC), SCOPE~\cite{}, BusTracker~\cite{ma2018query}), we observe that: (1) workloads are evolving over time, especially the value of parameters \hanxian{"parameter" or "attribute"? "parameter value" or "constant"? need to be unified in the whole paper} in the filter predicates. (2) A large portion (more than $93.3\%$) of the workload queries repeats frequently with only the filter parameters changed, \aka query templates (query with constants in the predicates removed) are re-occurring periodically. Especially, the daily templates are the majority in the workload as shown in Figure~\ref{fig:RecurringTemplates}. This gives us the opportunity to reuse the periodically recurring query templates. 

%Based on the aforementioned observations, we propose \sys, a holistic framework that effectively characterizes and forecasts evolving workloads to improve DBMS workload-dependent optimization techniques. %\sys\ utilizes a template-based representation to encode query statements and arrival time as a feature map, which is used for training and testing ML models. \sys\ employs a novel encoder-decoder ML model, \sysModel, to learn and predict future query templates, constants in the templates, and query arrival time. Additionally, \sys\ introduces a \cutNpack\ technique to cluster templates and train one ML model for each cluster, optimizing model capacity, prediction time, and storage efficiency. %The key contributions of \sys\ are summarized as follows:

\vspace{2mm}
\noindent\textbf{Contributions.} The paper makes the following contributions:
\squishlist
    \item %We qualitatively and quantitatively study on four real workloads and draw insights in terms of their re-occurrence, evolving patterns, and predictability, which motivates the design of \sys.
    %We conduct qualitative and quantitative studies on four real workloads, gaining insights into their re-occurrence, evolving nature, and predictability, which motivate the design of \sys.
    We conduct qualitative and quantitative studies on four real workloads (\S\ref{sec:motivation}), and found three crucial insights that motivate the design of \sys: 1) real workloads are highly recurrent (sharing the same \textit{query templates} but with different \textit{query parameters}); 2) these recurrent queries often exhibit time-evolving behavior; and 3) they are highly predictable.

    \item We propose and formally define two versions of the workload forecasting problem: next-$k$ (predicting the next $k$ queries in the future) and next-$\Delta t$ (predicting queries in the next $\Delta t$ time window), depending on whether the prediction window is number-based or time-based (\S\ref{sec:Problem}).

    %\item To the best of our knowledge, \sys\ is the first framework to identify and solve the future queries forecasting problem for time-evolving workload. \sys\ learns and forecasts the entire statements of future recurrent queries in various time spans with their corresponding arrival time. \tar{To the best of our knowledge, \sys\ is the first framework that learns and forecasts the \emph{entire} statements of future recurrent queries in various time spans with their corresponding arrival time.}
    
    %As mentioned above, previous work can only predict query arrival rate~\cite{ma2018query}, workload shifting~\cite{holze2008autonomic,holze2010towards} or recommend next query fragments with a blur range of constants~\cite{meduri2021evaluation}. Compared to query recommendation~\cite{meduri2021evaluation}, \sys\ provides a variety of forecasting horizons, which is adaptable by the applications. %\sys\ is valuable to improve the DBMS performance in multiple aspects and achieve autonomous DBMS.

    \item We propose an ML-based framework \sys\ to solve both versions of the query forecasting problem, while allowing some customization for the target application (\S\ref{sec:customization}). To the best of our knowledge, \sys\ is the first attempt to learn and forecast the \emph{entire} statements of future recurrent queries in various prediction windows with their corresponding arrival time for time-evolving workloads.

    \item For the next-$k$ forecasting problem, we propose a template-based featurization method to reuse recurrent query templates and better represent the time-evolving features (\S\ref{sec:featureEngineer}), and build an adapted encoder-decoder neural network, \sysModel, \textit{per template} for time-series learning and the multi-query prediction problem (\S\ref{sec:templatemodels}).

    \item To solve the next-$\Delta t$ forecasting problem, we extend the solution for the next-$k$ problem. The number of queries expected in the next $\Delta t$ time window varies a lot across templates. For templates with large expected numbers we need to `cut' them into sub-templates, in order to use the predicted next-$k$ queries to produce results for the next-$\Delta t$ problem. To reduce the number of models, we also `pack' templates with small expected number of queries into bins. After this \cutNpack algorithm (\S\ref{sec:cutNpack}), we build per-bin models (\S\ref{sec:perbinmodel}). This approach not only provides accurate results for the next-$\Delta t$ forecasting problem, but also reduces the number of \sysModel\ models by up to $23\times$, resulting in significant reduction in time and storage overhead by up to $13.6\times$ and $6.0\times$, respectively. 

    \item \sys\ provides a feedback loop to handle workload shifts, new emerging templates, and inactive templates (\S\ref{sec:feedbackloop}). It uses incremental learning to adapt the pre-trained \sysModel\ to shifted workloads, achieving accuracy comparable to full training, with only a few seconds of fine-tuning overhead.

    \item We evaluate \sys\ on four real workloads (\S\ref{sec:eval}) and demonstrate its accurate forecasting ability. Furthermore, we applied \sys\ to two real-world applications: materialized view selection and semantic caching of query results on \mssales\ and BusTracker workloads, respectively. Our results show up to $6.5\times$ improvement in view selection and $7.6\times$ improvement in semantic caching using forecasted workloads compared to historical workloads, highlighting the efficacy of \sys.

    
    %\item %To reuse the highly-recurrent templates, \sys\ deploys a template-based featurization. It wisely simplifies the forecasting problem compared to token-based featurization~\cite{jain2018query2vec,meduri2021evaluation} and generates well-formed query statements. It is more efficient and takes $13.8\times$ smaller feature maps storage overhead compared to bit-vector representation~\cite{meduri2021evaluation}.
  %  We propose a ML-based framework \sys\ to solve both versions of the query forecasting problem, consisting of (1) a tailored template-based featurization to reuse recurrent templates and better represent the time-evolving features. (2) \sysModel, an adapted encoder-decoder neural network for time-series learning and multi-query prediction problem, achieving an average $F1$ score of $86.9\%$.
    %employs a template-based featurization to reuse highly-recurrent templates, simplifying the forecasting problem compared to token-based featurization methods. It generates well-formed query statements and is more efficient, with $13.8 \times$ smaller storage overhead compared to token-basesd representation.

    %\item %We adapt the encoder-decoder architecture and propose \sysModel\ for time-series learning and multi-query prediction problem with an average accuracy of \todox{$xxx\%$}. We improve the framework scalability and reduce the number of \sysModel\ models to train for each workload with a template \cutNpack\ method and significantly improve time and storage efficiency by up to \todox{$xxx\times$}.
    
    %To solve the variable template trace length problem in real workloads, we propose a template \cutNpack\ approach to reorganize templates and reduce the number of \sysModel\ models by up to $23\times$, resulting in significant reduction on time and storage overhead by up to $13.6\times$ and $6.0\times$. 

    %\item %\sys\ provides a feedback loop to deal with workload shift and a mechanism to handle new emerging templates. Specifically, \sys\ leverages incremental learning to efficiently adapt the pre-trained \sysModel\ onto the shifted workloads, with \todox{$xxx\%$} accuracy improvement and \todox{$xxx\times$} less training time compared to re-train the models from scratch.

    %\sys\ provides a feedback loop to handle workload shifts and new emerging templates. It leverages incremental learning to efficiently adapt the pre-trained \sysModel\ onto shifted workloads, achieving almost the same accuracy as a full training process, with only a few seconds fine-tuning overhead.


    %\item  %We demonstrate the usefulness of \sys\ with two real applications: view selection and query results caching on  \mssales\ and \wmc\ real workloads, respectively and show up to 45\% improvement on \mssales\ and \todox{} on \wmc\ compared to the ones without foresting. \sys\ is valuable to improve the DBMS performance in multiple aspects and achieve autonomous DBMS.
    %We showcase the efficacy of \sys\ through two real-world applications: view selection and query results caching on \mssales\ and \wmc\ workloads, respectively. Our results reveal up to $6.5\times$ improvement on \mssales\ and $7.6\times$ on BusTracker compared to approaches without forecasting. %\sys\ is a valuable tool for enhancing DBMS performance in various aspects and enabling autonomous DBMS operations.
\squishend


%\sys\ first categorizes the parameters according to their predictability. Then \sys\ deploys a template-based representation to encode the whole query text as a feature vector, upon which ML models can be trained and tested. \sys\ learns and predicts evolving workloads by novel encoder-decoder ML models. Furthermore, \sys\ improves the prediction time and storage efficiency by clustering the templates. In each cluster, we learn one ML model to forecast the whole query text in the future consisting of templates and all the constants in the templates. We evaluate \sys\ on two applications: view materialization and indexing, on four real workloads (Windows Mission Control, SCOPE, BusTracker, MSSales) and show \todox{$xxx\%$} and \todox{$xxx\%$} improvement accordingly. We summarize our contributions as follows: \hanxian{emphasize our tech novelty}
%\begin{itemize}
%    \item We propose \sys\, a general query-based workload forecasting framework, which is valuable to improve the DBMS performance in multiple aspects and achieve autonomous DBMS.
%    \item We characterize and categorize four real workloads and draw insights in terms of the re-occurrence, evolution, and predictability for the evolving workloads.
%    \item We propose a novel encoder-decoder neural network to learn over the past workloads and forecast the future workloads as well as their arrival time preciously and efficiently, enhanced with the novel clustering method.
%    \item Experiments show effectiveness and improvement on view materialization and index selection compared to other state-of-the-art models. 
%\end{itemize}

%To the best of our knowledge, \sys\ is the first framework to identify and solve the future queries forecasting problem for time-evolving workload. \sys\ learns and forecasts the entire statements of future recurrent queries in various time spans with their corresponding arrival time. \tar{To the best of our knowledge, \sys\ is the first framework that learns and forecasts the \emph{entire} statements of future recurrent queries in various time spans with their corresponding arrival time.}

%\noindent\textbf{Outline}. The rest of this paper is organized as follows:    \S\ref{sec:motivation} elaborates our study on real workloads and shows our motivation.  \S\ref{sec:Problem} defines the query forecasting problem and \S\ref{sec:overview} gives an overview of \sys. \S\ref{sec:design-k} and \S\ref{sec:design-delta} detail the solutions for the next-$k$ queries forecasting and the next-$\Delta t$ forecasting problem. We offer applicable customization in \S\ref{sec:customization}. %,~\ref{sec:scalable} and~\ref{sec:opt}. 
%We show two selected applications in  \S\ref{sec:apps}, which are used in further evaluations and discussions in  \S\ref{sec:eval}.
%We present our evaluation in \S\ref{sec:eval}, discuss on related work in  \S\ref{sec:related} and conclude the paper in \S\ref{sec:conclusion}.




==> content/6-scalable.backup.tex <==
\section{Next-$\Delta t$ Forecasting Models}
\label{sec:design-delta}

%In the previous section, we discussed our approach to solving the next-$k$ forecasting problem. As illustrated in \S\ref{sec:Problem}, a more practical forecasting benefits DBMS applications is acquiring the future queries in the next time interval $\Delta t$. Now, 
Having the next-$k$ solution, we now address some of the challenges in adapting next-$k$ forecasting for next-$\Delta t$ forecasting.

%we now extend its solution to solve the more demanding next-$\Delta t$ forecasting problem. We first motivate the need for 

\subsection{Challenges}% in Adapting Next-$k$ Forecasting for Next-$\Delta t$ Forecasting}

\noindent\textbf{Challenge 1: A required forecasting size exceeds a feasible $k$.} For a given target time interval $\Delta t$, a naive approach would be to use the next-$k$ forecasting method (\S\ref{sec:design-k}) and set a $k$ sufficiently large so that $k \geq \sigma$, where $\sigma$ is the number of queries arriving in $\Delta t$ as defined in \textsc{Definition 3.2} (\S\ref{sec:Problem}). To be more specific, we refer the number of queries of template i ($temp_i$) in $\Delta t$ as its template size, denoted as $\sigma_i(\Delta t)$. %Specifically, we can first predict the next $k$ queries $q_{n+1}, q_{n+2}, \dots, q_{n+k}$ for each template. We then find the first predicted query $q_{n+m+1}$ that exceeds the $\Delta t$ window based on the predicted query arrival time, i.e., $t_{q_{n+m}} < t_{q_{n}} + \Delta t \leq t_{q_{n+m+1}}$, where $m+1 \leq k$. Finally, we return $q_{n+1}, q_{n+2}, \dots, q_{n+m}$ as the output for the next-$\Delta t$ queries of the template. \hanxian{this part is mentioned in S3.}
%To obtain the forecasted queries for the entire workload, we sort and merge the forecasted queries of all templates according to their predicted arrival times. 
However, it is not always practically feasible to fulfill $k \geq \sigma_i(\Delta t), \forall temp_i$. On the one hand, $k$ cannot be arbitrary large and it is fixed during model training and inference. On the other hand, real workloads can have large volumes of queries as show in Table~\ref{tab:4statistics}, while DBMS applications can deploy a large $\Delta t$, \eg 1 day, 1 week, which results in a large required number of queries to forecast in the next $\Delta t$.

%\tar{add a para that explains that we keep k fixed, and why it cant be too big or too small. also how we determine it or point to the relevant places where we discuss it. then the next two challenges will become clear}
The the output window size $k$ of ML models is usually decided empirically rather than arbitrarily chosen, considering several factors: (1) The practical factor is the machine resource limitation. A larger $k$ brings more computation complexity and memory overhead. Given a specific machine to deploy \sysModel\ and a workload with a certain size, the maximum feasible $k$ is decided and bounded by the machine resource~\todox{cite}. (2) The model accuracy degrades when arbitrarily increasing $k$, as it is harder for a model to capture the extremely long patterns. Today's state-of-the-art sequence-to-sequence learning models~\cite{devlin-etal-2019-bert,radford2019language} typically adopt a feasible $k \in [128, 1024]$. %Previous research~\todox{cite} attempt to enlarge $k$ to $\sim 4000$ with additional training tricks to maintain accuracy, but it is still not arbitrary large or not even able to cover the largest template with $10{,}500$ queries per day in WMC, as shown in Figure~\ref{fig:imbalanced}. 
(3) A larger k requires more training data, thus may lead to the problem of inadequate data available to support training. 
%This is particularly true for time-series data, where the length of the time series limits the number of possible forecasting windows. 
Therefore, a maximum feasible $k$ in \sys is decided carefully and empirical based on the available resources, workload sizes, and model accuracy expectation. 
%Thus $k$ is required to carefully decided rather than an arbitrary large value according to the applications. 
Once $k$ is decided, it is fixed during the whole training and inference process. A change of $k$ leads to a new model architecture and requires model retraining from scratch.

%Now since we keep $k$ fixed, 
Given $k$ is limited and fixed, %there are two challenges when adopting the next-$k$ solution. First, 
the required number of queries to forecast for next-$\Delta t$ can be larger than $k$. For example, a physical design tool requires the next one-day's queries to perform optimization, \ie $\Delta t= 1 day$.
%considering a target %time window of one day, i.e. 
%$\Delta t= 1 day$ (a common time interval for physical design tasks), 
As shown in Figure~\ref{fig:imbalanced}, the required forecasting window size for a large sized template can be up to $10{,}500$ to cover the next day's queries. In this case, directly applying the next-$k$ solution is problematic with the above discussed feasible setting of $k \in [128, 1024]$.
%First, the query arrival rates of different templates can vary significantly. 
%As illustrated in Figure~\ref{fig:imbalanced}, the largest template in the \wmc workload has on average $\sim 10k$ queries per day, while the smallest one only has $\sim 10$ queries. 
%When the target time window is one day, i.e. $\Delta t= 1 day$ (a common time interval for physical design tasks), the per-template model for the largest template has to predict $\sim 10k$ queries, assuming a stable daily query volumes. 
%However, even when trained on massive clusters of GPUs, today's sequence-to-sequence learning neural networks can typically maintain only a $512$ to $2048$ forecasting window size~\cite{devlin-etal-2019-bert}. 
%So, for real workloads, it is not always feasible to increase $k$ to cover all the queries in the next $\Delta t$ window.  
This leads to the \textit{first challenge}: addressing \textit{large templates}, \ie templates with a substantially larger number of expected queries than $k$ in the next $\Delta t$.

\noindent\textbf{Challenge 2: Per-template model solution is not efficient for small templates and not scalable.} Conversely, the \textit{second challenge} involves the long tail of \textit{small templates}, i.e., templates with a very limited number of expected queries in the next $\Delta t$. For instance, Figure~\ref{fig:imbalanced} shows there are $1{,}893$ templates, which is $87.8\%$ of all the templates, with fewer than $50$ queries per day, much smaller than a common setting of $k$, \ie $k \gg \sigma_{small\_temp}(\Delta t)$. Directly deploying the next-$k$ solution is inefficient because it does not make the best of the model capacity. Moreover, in real workloads, the number of templates can be quite large, as demonstrated in Table~\ref{tab:recurrence}. Training a model for each template is not scalable, resulting in a vast number of models to maintain and significant scaling overhead, as shown in Table~\ref{tab:estimatedPerModel}.

\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{figure/imbalance.pdf}
  \caption{An example from \wmc workload where the number of queries received per day is imbalanced}. %\rana{ I don't think you need to rephrase the proposed approach here again the Figure since you are not showing the bins. Removing this will give some space.} To address this, we propose splitting  larger templates and grouping smaller templates to fit the model forecasting window.%\yuanyuan{This figure needs to be changed} 
\vspace{-20pt}

  \label{fig:imbalanced}
\end{figure}



%We next discuss how we address these two challenges.


%Given the resources available on the machines, we first estimate the maximum possible forecasting window size~\todox{{cite}} and determine a feasible value of $k$, both of which are workload-independent constants. The algorithm involves two main operations:

\subsection{\cutNpack Algorithm}
We introduce a two-step algorithm called \cutNpack, to address the above two challenges correspondingly. In the first step, the algorithm cuts larger templates into smaller templates of size smaller or equal to $k$. Then, in the second step, it packs multiple templates with size smaller than $k$ together into a bin (a logical term denoting a group of templates) such that the size of the bin is bounded by the bin capacity $k$. We discuss the two steps in more detail below.

\subsubsection{Template Cutting} 
Template cutting is the process of splitting a group of queries for a template into sub-groups, \aka \textit{sub-templates}, so that each size of them is not greater than $k$. We cut templates based on the arrival time. Specifically, we divide the $\Delta t$ interval into sub-intervals and use them to divide the group of queries. For instance, considering $\Delta t =$ 1 day, if $k<\sigma_i(1 \ day)$ but $k \geq \sigma_i(half \ day)$, we can split the template into two sub-templates: one with queries arriving between [0:00, 12:00) of a day and the other with queries arriving between [12:00, 24:00) of a day. %The first sub-template captures all morning queries of a day, while the second captures all afternoon queries of a day. 
Intuitively, we can then treat each sub-template as a new template and train two separate per-template models for these two sub-templates, allowing each to learn the evolving patterns for its specific time interval. Combining the forecasted queries from both models will result in the forecasted queries for the entire day.

For template cutting, we need to estimate the number of queries that are going to arrive for a given template in next $\Delta t$, denoted as $\widetilde{\sigma_i}(\Delta t)$. We discuss in the next subsection (\S\ref{sec:tempalteSize}) how we perform the estimation. We also choose a sufficiently fine-grained time window $\Delta t'$ of $\Delta t$ since we cut the interval into smaller sub-intervals. %that can be set based on the tuning interval at which performance is optimized. 
For example, if $\Delta t$ = 1 day, we may pick $\Delta t'$ = 1 hour.
%We find that $\Delta t'$ = 1 hour is reasonably small for most tuning applications. \hanxian{this is not true. eg for auto tuning we have minute granualarity}
We first use $\widetilde{\sigma_i}(\Delta t)$ to identify templates with sizes greater than $k$. For each such template, we examine the finer time granularity $\Delta t'$ and find the cutting points of sub-templates in the boundary of finer time intervals.
%The boundary of each finer time interval can be used as a cutting point of sub-templates. 
As depicted in Algorithm~\ref{algo:cutting}, the algorithm begins with the first $\Delta t'$ interval and greedily searches for a cutting point that results in the largest sub-template with a size less than $k$ by utilizing the estimated $\widetilde{\sigma_i}(\Delta t')$. After the cut is made, it moves on iteratively to search for the next cutting point of the next sub-template.

\begin{algorithm}
\caption{Template Cutting Algorithm}
\label{algo:cutting}
\begin{algorithmic}[1]
\State Input: $k$; $\widetilde{\sigma}_i(\Delta t')$ and $\widetilde{\sigma}_i(\Delta t)$ for template $temp_i$. 
\State Initialize the final sub-template set $S=\emptyset$. 
\For {$temp_i$ in all templates}
    \State Initialize the sub-template set for $temp_i: s_i=\emptyset$
    \If {$\widetilde{\sigma}_i(\Delta t) > k$}  
        \State Current\_sub\_template  $C=\emptyset$
        \State Current\_remaining\_size $R=k$
        \For{$\Delta t'_j$ in $\Delta t$}
            \If  {$\widetilde{\sigma}_i(\Delta t') \leq R$}
                \State \textcolor{gray}{\# fit into the current sub-template}
                \State $C = C \cup \{temp_i(\Delta t'_j)\}, \ R=R-\widetilde{\sigma}_i(\Delta t')$
            \Else
                \State \textcolor{gray}{\# initialize a new sub-template}
                \State $s_i = s_i \cup \{C\}$
                \State $C=\{temp_i(\Delta t'_j)\},R=k-\widetilde{\sigma}_i(\Delta t'_j)$
                
        
            \EndIf
        \EndFor 
    \Else
        \State $s_i=\{temp_i\}$
    \EndIf
    \State $S = S\cup s_i$
\EndFor

\State Output: the final sub-template set $S$ %, $s.t. k \geq \sum_{i \in s_j} \hat{\sigma}_i(\Delta t'), \forall s_j \in S$
\end{algorithmic}
\end{algorithm}


\subsubsection{Template Packing}
%After cutting, the sizes of all templates are smaller than $k$.\tar{unclear why? we used k to cut the templates why would they be smaller than k. }
As mentioned in \textit{Challenge 2}, there may be many templates in the workload with very small sizes. We `pack' multiple such smaller templates into bins such that the total number of expected queries per bin is no larger than $k$. %, \ie $k \geq \sum_i(\sigma_i(\Delta t)), \forall i \in bin_j, \forall bin_j$. %In addition to the typical bin-packing constraints, such as not exceeding the $k$ and assigning every template to exactly one bin, 
When packing the small templates into bins, we also considering the number of templates per bin, \ie we avoid aggressively packing too many small templates in a bin.
%we also add a constraint that limits the maximum number of templates per bin to a constant $d$. 
This is necessary because each bin can contain queries from multiple templates, and the per-bin model predicts the template, parameter values, and arrival time for each future query. If there are too many templates to predict, the model's accuracy suffers on the complicated patterns combining of various template patterns. Quantitatively, we set the maximum number of templates per bin to a constant $d$ to alleviate this problem. 
%Having a cap $d$ helps alleviate this problem. 
The $d$ controls the degree of `packing' and brings a trade-off: a smaller $d$ may leads to a higher model accuracy but can result in more bins and thus more models to train.  
Empirically, we set $d=50$ in \sys, as it results in adequately accurate models for our workloads. We formulate this packing process as an integer linear programming problem:% constrained optimization problem:

\begin{comment} %this is a simpler version - but not super formal
\begin{equation*}
\begin{aligned}
& \text{minimize} \ \ &&\#bins \\
& \text{subject to} 
&&  \sum_i(\widetilde{\sigma}_i(\Delta t)) \leq k, \ \forall temp_i \in bin_j, \ \forall bin_j  \\
& && \#templates\_in\_bin_j \leq d,  \ \forall bin_j  
\end{aligned}
\end{equation*}
\end{comment}



\begin{equation*}
\begin{aligned}
& \text{minimize} \ \ &&\#bins = \sum_j y_j \\
& \text{subject to} 
    && \#bins \geq 1\\
&    &&  \sum_{i \in bin_j}(\widetilde{\sigma}_i(\Delta t)) \leq k, \ \forall temp_i \in bin_j, \ \forall bin_j  \\ %not exceeding k
&   && \#templates\_in\_bin_j \leq d,  \ \forall bin_j  \\
& && \sum_j x_{ij} =1, \forall temp_i \\ %assigning every template to exactly one bin
& && y_j, x_{ij} \in \{0,1\}, \forall temp_i, bin_j
\end{aligned}
\end{equation*}

Where $y_j=1$ if bin j is used and $x_{ij}=1$ if template $i$ is put into bin $j$. To find such a partition of all the small templates into disjoint bins, we modified a classical greedy bin-packing algorithm~\cite{martello1990knapsack} to solve this problem by preferring a bin with fewer templates when multiple bins can fit a template. It is worth mentioning that, after \cutNpack, the bins are usually not fully occupied (\ie with sizes smaller than k), which allows accurately forecasting even with normal minor variations of template size in real workloads. \tar{do we evaluate the right size of d?}\hanxian{we did not evaluate d in S9. We just mentioned an empirical number here.}

\subsubsection{Per-Bin Models}\label{sec:perbinmodel}
%\section{Improving Scalability}\label{sec:scalable}

%The per-template model is sufficient to solve the next-k query forecasting problem for small size workload. However, there are two main challenges in scaling up the per-template model to real workloads: (1) Efficient training on large query volumes: As shown in Table~\ref{tab:4statistics}, the daily volume of queries amounts to millions, which result in an enormous amount of training data. Enabling efficient model training and fine-tuning %and improving scalability of the forecasting framework 
%to accommodate such large query volumes, are critical for practical deployment in real-world workloads. Previous paper~\cite{ma2018query} performs down-sampling and heavily reduces the dataset volume by $\sim 14k \times$ by only counting the number of queries per minute, which is target on query arrival rate forecasting. However, in the query workload forecasting problem, we aim to predict the exact query statement in the upcoming sequence. Any downsampling skews the time-evolving patterns and biases the data distribution, resulting in forecasting accuracy sacrifice. With the long query traces and the large number of templates in the real workloads, the training time and storage overhead for the per-template models linearly scale up as shown in Table~\ref{tab:estimatedPerModel}. This calls for optimizing the model capacity and minimizing the number of models to train.



%(2) Another challenge is the number of query for templates are imbalanced, as shown in Figure~\ref{fig:imbalanced}. The large-volume template can have $\sim 10k$ queries per day, while the small one only has $\sim 10$. Since one of our target applications is view selecting, which is performed at a daily frequency. It is required that our models are capable of predicting the future queries for a one-day volume in a single forecasting, \aka the next time-interval forecasting, which requires a $\sim 10k$ forecasting window size. However, even trained on massive clusters of GPUs, today's sequence-to-sequence learning neural networks can typically only maintain a $512$ to $2048$ forecasting window size~\cite{}. 
%In our study and experiment, we figured out that the designed \sysModel\ has good scalability -- when scaling up input and output length and scaling up the forecasting window size, as shown in Section~\ref{sec:eval}. However, given the computation and memory resource constraints of the machine on which we train our models, it is not feasible to always increase the forecasting window size to fit the increasing-size workloads. Moreover, we observe there are a large number ($\sim 17500$) of small templates with fewer than $25$ queries per day. It is inefficient to train a large number of per-template models for all the small templates. To improve the time and storage efficiency and deal with the huge templates, we propose to \cutNpack\ the templates into bins according to the model forecasting window size, the volume of templates, and the target applications. Based on the new bins, we adjust the pre-template model to the pre-bin model, \ie learn each model to forecast future queries for all the templates in the next time interval for each bin. We now describe the \cutNpack\ approach.


%Based on our observation, the recurrent templates have a stable number of queries per day. Thus we use the average number of queries per day to approximate the number of queries in the next day. Given the prediction window size $m$ and the average number of queries $\sigma_i$ per day for each template $i$, we group the templates into one bin, or divide one large template into separate bins, so that one prediction $m$ can cover the prediction for the next time interval for all the templates in a bin: $m \geq \sum_{i \in c_j} \sigma_i, \forall c_j$. Specifically, \textbf{Cut:} We cut the big templates into smaller time-interval bins so that one forecasting can cover the next time-interval. For example, the original observation time interval is one day. For a large template, we can divide a template into two sub-templates with the AM and PM time frames, or divide it into three sub-templates with smaller time intervals 0AM-8AM, 8AM-16PM, 16PM-12AM, \etc so that the forecasting window size can cover the sub-templates. \textbf{Pack:} We pack the small templates into larger volume bins to reduce the number of models to train and improve the training efficiency. We solve the bin-packing problem by greedily packing more templates as possible as long as one forecasting can cover the next interval queries in a bin. We show the detail of the \cutNpack\ in Algorithm~\ref{algo:clustering}. 



%Another large-volume issue is the prediction volume problem. Since our target application is view selecting, which is performed at a daily frequency. It is required that our models can predict one day volume's future queries at a time. This corresponds to $\sim 10,000 / 43,000 / 44,000$ queries per day for WT / SCOPE / BusTracker. It is difficult to build such a forecasting model to predict such a large volume at a time. To solve this challenge, \sys\ first proposes to train one model to predict for one template, and later proposes to cluster various workloads based on the workload features and adjust the pre-template model to the pre-cluster model to improve model efficiency. The per-template model is sufficient to solve the next-k query forecasting problem for small size workload. However, given the long query traces and a large number of templates in the real workloads (Table~\ref{tab:4statistics}), it is not efficient and not scalable to build and manage each model for each template. To further improve the time and storage efficiency, we propose to \cutNpack\ the templates into bins according to the capacity of models, volume of templates, and the target applications. Based on the new bins, \sys\ is able to adjust the pre-template model to the pre-cluster model, \ie learn each model to forecast for all the templates in one bin, thus reducing the total number of models to train and maintain and improve model efficiency. Now we discuss our \cutNpack\ algorithm. 


%Taking view selection as an example target application, it is required that the forecaster predicts all the future workloads that are needed by the next view selection interval. A common interval example to perform view selection is one day~\cite{}, and it is required that the models can predict all the next day's queries by the end of today before applying view selection and future queries come. To make \sys\ practical to view selection, we design our template distribution method based on the prediction window size of the models and the average numbers of queries of the templates, to both make the best of ML models capacity and fulfill the practical requirement.


%Based on our observation, the recurrent templates have a stable number of queries per day. %study in Section~\ref{sec:motivation}, the daily templates are the majority of the workload, and they have a very stable number of queries per day \todox{need to add this part in Sec 2} %\yuanyuan{Do you think we should consider building a model to predict the number of queries in the future time window for a template, and use that as the input for Algorithm 1 when deciding how to cut and pack tempates?}. 

After cutting and packing templates into bins, we now adapt the per-template models into per-bin models to solve the next-$\Delta t$ forecasting problem. We still use the \sysModel as the forecasting models, but have to make the following adaptations:

\squishlist
\item \textbf{The feature map} is more complex for a per-bin model, since it includes queries from all templates or sub-templates within a bin, rather than just one template. To account for multiple templates within each bin during featurization, it is necessary to include the template ID as a feature and the feature map must also encompass the parameter values from all templates within the bin.

\item 
\textbf{The forecasting task} becomes more challenging when modeling a mixed time-series pattern of various templates in a bin, as opposed to the pattern of a single template. The per-bin model must accurately forecast the template ID and all parameter values within the bin, to ensure that the predicted query can be correctly reconstructed with the appropriate template and parameter values.

%\item \textbf{The online feedback loop} is also improved. It is crucial to not only monitor model accuracy, fine-tune models, and detect new and inactive templates, but also to keep track of the size of each template. If the total size of templates exceeds the bin capacity, it becomes necessary to re-adjust the assignment of templates to bins and re-train the models for changed bins. 
\squishend

%With template \cutNpack, we adjust the per-template models to per-bin models by adapting the following aspects: (1) In preprocessing, we first \cutNpack\ the templates and build one feature map for each bin. (2) Instead of using one feature map to encode one template, we expand the feature map to encode all the attributes of all the templates in a bin. (3) We include the template ID so that the model can also forecast which template ID will come next in a bin. (4) When reconstructing the forecasted query, we refer to the template context by the template ID, and then fill the corresponding parameters into the template. %When constructing the feature map, if one attribute appears in the template, the featurization is the same as discussed in Section~\ref{sec:featurization}. Otherwise we set it as a special categorical value $\$$, as shown in Figure~\ref{fig:per_cluster_temp2}
%We deploy the per-bin models to solve the next time interval forecasting problem. We identify the forecasted queries for the next time interval by the forecasted arrival time.

\subsection{Estimating Template Size}\label{sec:tempalteSize}
We now discuss how to estimate the template size that we use for template cutting. To address this, we train an additional one-layer LSTM to forecast it.
We collect $\sigma_i(\Delta t')$ in the historical workload as a time series to train the LSTM model to forecast the future arrival rates in the $\Delta t'$ granularity (introduced earlier), denoted as $\hat{\sigma_i}(\Delta t')$.  Using $\hat{\sigma_i}(\Delta t')$, we can then compute $\hat{\sigma_i}(\Delta t)$. To ensure our next-$\Delta t$ forecasting models can stably predict multiple successive $\Delta t$ windows without costly retraining, we also set a longer forecasting horizon $\Delta T$, e.g., $\Delta T$ = 1 week given $\Delta t$ = 1 day. This provides a longer preview (e.g., $\Delta T = 7 \Delta t$) of future arrival rates. We then conservatively use the upper-bound of all forecasted $\hat{\sigma_i}(\Delta t)$ to approximate the template size in the next $\Delta t$, i.e., $\widetilde{\sigma_i}(\Delta t)=\max(\hat{\sigma}_i(\Delta t_j)), \forall \Delta t_j \in \Delta T$. Similarly, we can approximate the template size within each $\Delta t'$ of $\Delta t$ as $\widetilde{\sigma_i}(\Delta t')=\max(\hat{\sigma}_i(\Delta t'_j)), \forall \Delta t'_j \in \Delta T$.

Note that this one-layer LSTM model is only used to estimate the size of a template for the \cutNpack algorithm. The forecasted arrival time from \sysModel still determines the actual number of queries in the next-$\Delta t$ prediction. Note that while one-layer LSTM model is sufficient for our intended purpose, we can also use QueryBot\_5000~\cite{ma2018query} to estimate the template size. In our study over the four workloads, we have observed that when the time interval $\Delta t$ is coarse, such as 1 day, the majority of templates exhibit stable query rates. In such cases, we can even approximate the template size using the upper-bound of the historical rate.


%, we first identify whether a template is large enough and requires to be cut into smaller sub-templates. We care in the next forecasting, whether the forecasting window size $k$ can cover the number of queries in the next $\Delta t$, denoted as $\sigma_i(\Delta t)$ for template $i$. Given a specific machine to deploy \sysModel\ with a certain resource and given a workload with a certain workload size, we can estimate the upper bound of forecasting window size~\todox{{cite}} and decide a feasible $k$ for \sysModel. To better estimate the query arrival rate in the future $\Delta t$ windows for each template in advance, we train an additional one-layer LSTM to forecast it. We first pick a sufficiently finer granularity time window $\Delta t'$ of $\Delta t$. For example, if $\Delta t$= 1 day, we may pick $\Delta t'$ = 1 hour. We collect $\sigma_i(\Delta t')$ in the historical workload in a time series to train the LSTM model to forecast the future arrival rate in the $\Delta t'$ granularity, which will be used to help template cutting later in Algorithm~\ref{algo:cutting}. We set a larger forecasting horizon $\Delta T$, \eg $\Delta T$ = 1 week given $\Delta t$ = 1 day.%Every time we leverage the model to forecast for the next $\Delta T$ horizon, where $\Delta T$ is a larger time interval, \eg $\Delta T$=1 week, 
%which gives us a longer preview (\eg $\Delta T = 7 \Delta t$s) of future arrival rates. Then we conservatively use the the upper-bound of the forecasted $\sigma_i(\Delta t)$, denoted as $max(\hat{\sigma}_i(\Delta t)), \forall \Delta t \in \text{the next } \Delta T$, to approximate the template size in the next $\Delta t$, since we want to make sure the forecasting can be covered by $k$. Then we compare it with $k$ and cut the template if it is over $k$.
%is over $k$. If so, we identify it as a large template and need to cut it. 
%This LSTM model is fine-tuned periodically to improve accuracy. This LSTM model is only used to identify large templates to be cut. The actual number of queries in the next-$\Delta t$ forecast are stilled identified by the forecasted arrival time. For the four workloads that we studied, we have observed that when $\Delta t$ is coarse, such as 1 day, most of the templates have stable query rates. In this case, we can also simply use the upper-bound of the historical rate to approximate the template size. 



\iffalse
\subsection{The \cutNpack Algorithm}

We now introduce the \cutNpack algorithm to address both challenges of the next-$\Delta t$ problem. After selecting a machine to deploy \sysModel, along with the specific resource configurations, and given a workload of a certain size, we can estimate the maximum possible forecasting window size~\todox{{cite}} and then determine a feasible value of $k$ for \sysModel. 
To deal with the first challenge brought by the templates with size greater than $k$, the \cutNpack algorithm `cuts' them into \textit{sub-templates} such that each sub-template has a size less than $k$. Then it `packs' the resulting sub-templates along with other un-cut templates into bins, to reduce the number of models that need to be built. 

%\subsection{Large Template Size Challenge}
%As mentioned in \S~\ref{sec:Problem}, in practice, it is difficult to determine the number of queries $k$ to forecast in advance; rather, a more practical version of problem is to forecast the future queries for the next time interval $\Delta t$ to help database tuning tools. 
%The key challenge here is that we do not know how many queries to predict. 
%In an ideal case where $k$ is sufficiently large, we can first predict the next $k$ queries $q_{n+1}, q_{n+2},...q_{n+k}$ for each template. Then, we find the first predicted query $q_{n+m+1}$ that exceeds the $\Delta t$ window based on the predicted query arrival time, i.e., $t_{q_{n+m}}<t_{q_{n}}+\Delta t \leq t_{q_{n+m+1}}$ where $m+1\leq k$. Finally, we return $q_{n+1}, q_{n+2},...q_{n+m}$ as the output for the next-$\Delta t$ queries of the template. To get the forecasted queries for the entire workload, we aggregate the forecasted queries of all templates and sort-merge queries based on the predicted arrival time.


\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{figure/imbalance.pdf}
  \caption{An example from \wmc workload where the number of queries received per day is imbalanced}. %\rana{ I don't think you need to rephrase the proposed approach here again the Figure since you are not showing the bins. Removing this will give some space.} To address this, we propose splitting  larger templates and grouping smaller templates to fit the model forecasting window.%\yuanyuan{This figure needs to be changed} 
\vspace{-20pt}

  \label{fig:imbalanced}
\end{figure}

%Unfortunately, this ideal case is rare in practice. The query arrival rates of different templates vary a lot. As shown in Figure~\ref{fig:imbalanced}, the largest template in the \wmc workload can have on average $\sim 10k$ queries per day, while the smallest one only has $\sim 10$ queries. If the target time window is one day, i.e. $\Delta t= 1 day$, which is a common time interval for physical design tasks, such as materialized view recommendation, the per-template model for the largest template has to predict $\sim 10k$ queries. However, even trained on massive clusters of GPUs, today's sequence-to-sequence learning neural networks can typically only maintain a $512$ to $2048$ forecasting window size~\cite{devlin-etal-2019-bert}. So, for real workloads, it is not always feasible to increase $k$ to cover forecasting all the queries in the next $\Delta t$ window. 
%Thus we propose to \textbf{cut} the large templates whose number of queries per target time window is greater than a feasible $k$.

%\hanxian{I removed the additional model to forecast the arrival rate. Since in the offline stage, we can measure the templates size rather than estimating them.}




%To start, we first identify whether a template is large enough and requires to be cut into smaller sub-templates. We care in the next forecasting, whether the forecasting window size $k$ can cover the number of queries in the next $\Delta t$, denoted as $\sigma_i(\Delta t)$ for template $i$. Given a specific machine to deploy \sysModel\ with a certain resource and given a workload with a certain workload size, we can estimate the upper bound of forecasting window size~\cite{cite a paper on how to estimate it} and decide a feasible $k$ for \sysModel. To better estimate the query arrival rate in the future $\Delta t$ windows for each template in advance, we train an additional one-layer LSTM to forecast it. We first pick a sufficiently finer granularity time window $\Delta t'$ of $\Delta t$. For example, if $\Delta t$= 1 day, we may pick $\Delta t'$ = 1 hour. We collect $\sigma_i(\Delta t')$ in the historical workload in a time series to train the LSTM model to forecast the future arrival rate in the $\Delta t'$ granularity, which will be used to help template cutting later in Algorithm~\ref{algo:cutting}. We set a larger forecasting horizon $\Delta T$, \eg $\Delta T$ = 1 week given $\Delta t$ = 1 day.%Every time we leverage the model to forecast for the next $\Delta T$ horizon, where $\Delta T$ is a larger time interval, \eg $\Delta T$=1 week, 
%which gives us a longer preview (\eg $\Delta T = 7 \Delta t$s) of future arrival rates. Then we conservatively use the the upper-bound of the forecasted $\sigma_i(\Delta t)$, denoted as $max(\hat{\sigma}_i(\Delta t)), \forall \Delta t \in \text{the next } \Delta T$, to approximate the template size in the next $\Delta t$, since we want to make sure the forecasting can be covered by $k$. Then we compare it with $k$ and cut the template if it is over $k$.
%is over $k$. If so, we identify it as a large template and need to cut it. 
%This LSTM model is fine-tuned periodically to improve accuracy. This LSTM model is only used to identify large templates to be cut. The actual number of queries in the next-$\Delta t$ forecast are stilled identified by the forecasted arrival time. For the four workloads that we studied, we have observed that when $\Delta t$ is coarse, such as 1 day, most of the templates have stable query rates. In this case, we can also simply use the upper-bound of the historical rate to approximate the template size. 



\subsubsection{Template Cutting} 

When we refer to cutting a template, we mean dividing the group of queries for a template into sub-groups, which we call \textit{sub-templates}. It's important to note that queries in the sub-template share the same query template as the queries in the original template. There are various methods to cut a template. To maintain the time series aspect of the problem, we cut templates based on the arrival time. Specifically, we divide the $\Delta t$ interval into sub-intervals and use them to divide the group of queries. For instance, if $\Delta t = 1 day$, we can split the template into two sub-templates based on query arrival times: one with queries arriving between [0:00, 12:00) of a day and the other with queries arriving between [12:00, 24:00) of a day. The first sub-template captures all morning queries of a day, while the second captures all afternoon queries of a day. Intuitively, we can train separate models for the two sub-templates, allowing each to learn the evolving patterns for its specific time interval. Combining the forecasted queries from both models will result in the forecasted queries for the entire day.

The process of cutting templates is outlined in Algorithm~\ref{algo:cutting}. First, we use the estimated $\widetilde{\sigma_i}(\Delta t)$ to identify templates with sizes greater than $k$. For each such template, we examine the finer time granularity $\Delta t'$ as introduced in \S\ref{sec:tempalteSize}. The boundary of each finer time interval can be used as a cutting point. The algorithm begins with the first $\Delta t'$ interval and greedily searches for a cutting point that results in the largest sub-template with a size less than $k$ by utilizing the estimated $\widetilde{\sigma_i}(\Delta t')$. After the cut is made, it moves on iteratively to search for the next cutting point.


%The high-level idea is to split the queries of a large size template according to their arrival time into smaller sub-templates (smaller groups), such that each sub-template has a total number of queries per $\Delta t$ that is less than $k$. With the LSTM model to forecast the $\hat{\sigma}_i(\Delta t'_j)$, 
%We estimate the number of queries of a template $i$ per time window $\Delta t$, denoted as $\sigma_i(\Delta t)$. We pick a sufficiently finer granularity time window $\Delta t'$ of $\Delta t$ so that $\sigma_i(\Delta t') \leq k$, to help further template cutting. For example, if $\Delta t =$ 1 day, we may pick $\Delta t'=$ 1 hour. 
%we can now identify the large templates and group the queries in each $\Delta t'_j$ into sub-templates according to their size and $k$. We did not perform arbitrary grouping. Instead, we prefer to group the queries with continuous arrival time into the same sub-template for a time-series forecasting, as discribed in Algorithm~\ref{algo:cutting}. 

After cutting the template, we end up with multiple sub-templates, each of which has a size that is smaller than $k$. We can then treat each sub-template as if it were a new template.

%We calculate the query arrival rate per $\Delta t'$ window for each template, and build a simple one layer LSTM model to predict the arrival rate for the next $l$ windows, where $l$ is sufficiently large for a time interval of periodic fine-tuning %\tar{is this the first time we mentioned of periodic re-adjustment? If so, maybe add a line to explain what it means.} 
%of models. To define the size of the template for a $\Delta t_j$ window, denoted as $\sigma(temp_i(\Delta t_j))$, we can use the upper bound of the query rate for the $\Delta t$ window based on the predictions. We have observed that when $\Delta t$ is coarse, such as one day, most of the templates in our four real workloads have stable query rates. In this case, we can use the upperbound of the historical rate as the template size.

%\textbf{Cut.} In order to handle a large template, we can divide it into smaller sub-templates such that each sub-template has a size that is less than $k$. The division is based on the query arrival time. For instance, if $\Delta t = 1 day$, we can split the template into two sub-templates based on query arrival times: one with queries between [0:00, 12:00) and another with queries between [12:00, 24:00). If any of the sub-template still has the size greater than $k$, then we recursively perform cutting. The number of cuts and the actual cutting points are determined based on the size of the sub-templates, which can be estimated using the arrival rate prediction discussed earlier. After dividing the template, we end up with multiple sub-templates, each of which has a size that is smaller than $k$. We can then treat each sub-template as a new template.

\begin{algorithm}
\caption{Template Cutting Algorithm}
\label{algo:cutting}
\begin{algorithmic}[1]
\State Input: $k$; $\widetilde{\sigma}_i(\Delta t')$ and $\widetilde{\sigma}_i(\Delta t)$ for template $temp_i$. 
\State Initialize the final sub-template set $S=\emptyset$. 
\For {$temp_i$ in all templates}
    \State Initialize the sub-template set for $temp_i: s_i=\emptyset$
    \If {$\widetilde{\sigma}_i(\Delta t') > k$}  
        \State Current\_sub\_template  $C=\emptyset$
        \State Current\_remaining\_size $R=k$
        \For{$\Delta t'_j$ in $\Delta t$}
            \If  {$\widetilde{\sigma}_i(\Delta t') \leq R$}
                \State \textcolor{gray}{\# fit into the current sub-template}
                \State $C = C \cup \{temp_i(\Delta t'_j)\}, \ R=R-\widetilde{\sigma}_i(\Delta t')$
            \Else
                \State \textcolor{gray}{\# initialize a new sub-template}
                \State $s_i = s_i \cup \{C\}$
                \State $C=\{temp_i(\Delta t'_j)\},R=k-\widetilde{\sigma}_i(\Delta t'_j)$
                
        
            \EndIf
        \EndFor 
    \Else
        \State $s_i=\{temp_i\}$
    \EndIf
    \State $S = S\cup s_i$
\EndFor

\State Output: the final sub-template set $S$ %, $s.t. k \geq \sum_{i \in s_j} \hat{\sigma}_i(\Delta t'), \forall s_j \in S$
\end{algorithmic}
\end{algorithm}



%\subsection{Scalability Issue}
%\label{sec:scalability}

%On the flip side of the coin, we often observe a long tail of small templates in real workloads. For example, Figure~\ref{fig:imbalanced} shows $1893$ templates with fewer than $50$ queries per day. In real workload, the number of template can be a very huge number as shown in Table~\ref{tab:recurrence}. It is inefficient and not scalable to simply train a per-template model for each template, which results in an enormous number of models to maintain and a scaling-up overhead as shown in Table~\ref{tab:estimatedPerModel}. 
%\tar{I think the last point is less related to $\Delta t$ forecasting, but more of a scalability issue?}


\subsubsection{Template Packing}
After cutting, the sizes of all templates are smaller than $k$.\tar{unclear why? we used k to cut the templates why would they be smaller than k.}
But, we may also end up with lots of very small templates. To address this issue issue, we propose to `pack' the queries from multiple templates into bins and ensure that $k$ can still cover the total number of expected queries for the templates in each bin for the next $\Delta t$ time interval. After packing, we can train a \sysModel per bin to solve the next-$\Delta t$ forecasting problem. 

We formulate this packing process as a bin-packing problem,, where each bin has a capacity of $k$. In addition to the typical bin-packing constraints, such as not exceeding the bin's capacity and assigning every template to exactly one bin, we also add a constraint that limits the maximum number of templates per bin to $d$. This is necessary because each bin can contain queries from multiple templates, and the per-bin model needs to predict the template, parameter values, and arrival time for each future query. If there are too many templates to predict, the model's accuracy may suffer. Having a cap $d$ helps alleviate this problem. Empirically, we set $d=50$ in \sys, as it results in adequately accurate models for our workloads. We modified a classical greedy bin-packing algorithm~\cite{martello1990knapsack} to solve this bin-packing problem by preferring a bin with fewer templates when multiple bins can fit a template.



%Each bin now can contain queries from multiple templates

%To address the scalability issue, we propose to \textbf{pack} the queries from small templates into bins and ensure the forecasting window size $k$ can still cover the total number of queries for the next $\Delta t$ time interval. 


%To tackle the challenges from both large templates and small templates, we propose to \cutNpack templates to reorganize workload queries into bins. 

%Similar to the per-template models, we can next train \textit{per-bin} models to solve the next-$\Delta t$ forecasting problem. %The goal of the \cutNpack algorithm is to make sure given the target $\Delta t$ and a computationally feasible $k$ value based on the available resources for model training, $k$ is big enough such that the next-$k$ queries predicted from each per-bin model cover all the queries needed for the next-$\Delta t$ time window. 



%\subsection{\cutNpack Algorithm}\label{sec:cutNpack}
%The high-level idea of the \cutNpack algorithm is to \textit{cut} large templates and \textit{pack} small templates into bins, so that each per-bin model has the adequate capacity for the next-$\Delta t$ forecasting problem, given a feasible value $k$. 

%To start, we need to measure the size of a template for a given time window $\Delta t$. We first pick a sufficiently finer granularity time window $\Delta t'$ of $\Delta t$. For example, if $\Delta t = 1 day$, we can pick $\Delta t'=1 hour$. 
%We calculate the query arrival rate per $\Delta t'$ window for each template, and build a simple one layer LSTM model to predict the arrival rate for the next $l$ windows, where $l$ is sufficiently large for a time interval of periodic fine-tuning %\tar{is this the first time we mentioned of periodic re-adjustment? If so, maybe add a line to explain what it means.} 
%of models. To define the size of the template for a $\Delta t_j$ window, denoted as $\sigma(temp_i(\Delta t_j))$, or simply $\sigma_i$ if there is no ambiguity, we can use the upper bound of the query rate for the $\Delta t$ window based on the predictions. We have observed that when $\Delta t$ is coarse, such as one day, most of the templates in our four real workloads have stable query rates. In this case, we can use the upperbound of the historical rate as the template size.

%\textbf{Cut.} In order to handle a large template, we can divide it into smaller sub-templates such that each sub-template has a size that is less than $k$. The division is based on the query arrival time. For instance, if $\Delta t = 1 day$, we can split the template into two sub-templates based on query arrival times: one with queries between [0:00, 12:00) and another with queries between [12:00, 24:00). If any of the sub-template still has the size greater than $k$, then we recursively perform cutting. The number of cuts and the actual cutting points are determined based on the size of the sub-templates, which can be estimated using the arrival rate prediction discussed earlier. After dividing the template, we end up with multiple sub-templates, each of which has a size that is smaller than $k$. We can then treat each sub-template as a new template.
%\tar{we may want to talk about how we perform merging after predictions? We need the whole queries for views, etc.}

%\textbf{Pack.} After cutting, the sizes of all templates are smaller than $k$. But, we may also end up with lots of very small templates. We apply a greedy bin-packing algorithm~\cite{martello1990knapsack} to pack templates into bins, each of which has a size $k$. 


\subsection{Per-Bin Models}\label{sec:perbinmodel}
%\section{Improving Scalability}\label{sec:scalable}

%The per-template model is sufficient to solve the next-k query forecasting problem for small size workload. However, there are two main challenges in scaling up the per-template model to real workloads: (1) Efficient training on large query volumes: As shown in Table~\ref{tab:4statistics}, the daily volume of queries amounts to millions, which result in an enormous amount of training data. Enabling efficient model training and fine-tuning %and improving scalability of the forecasting framework 
%to accommodate such large query volumes, are critical for practical deployment in real-world workloads. Previous paper~\cite{ma2018query} performs down-sampling and heavily reduces the dataset volume by $\sim 14k \times$ by only counting the number of queries per minute, which is target on query arrival rate forecasting. However, in the query workload forecasting problem, we aim to predict the exact query statement in the upcoming sequence. Any downsampling skews the time-evolving patterns and biases the data distribution, resulting in forecasting accuracy sacrifice. With the long query traces and the large number of templates in the real workloads, the training time and storage overhead for the per-template models linearly scale up as shown in Table~\ref{tab:estimatedPerModel}. This calls for optimizing the model capacity and minimizing the number of models to train.



%(2) Another challenge is the number of query for templates are imbalanced, as shown in Figure~\ref{fig:imbalanced}. The large-volume template can have $\sim 10k$ queries per day, while the small one only has $\sim 10$. Since one of our target applications is view selecting, which is performed at a daily frequency. It is required that our models are capable of predicting the future queries for a one-day volume in a single forecasting, \aka the next time-interval forecasting, which requires a $\sim 10k$ forecasting window size. However, even trained on massive clusters of GPUs, today's sequence-to-sequence learning neural networks can typically only maintain a $512$ to $2048$ forecasting window size~\cite{}. 
%In our study and experiment, we figured out that the designed \sysModel\ has good scalability -- when scaling up input and output length and scaling up the forecasting window size, as shown in Section~\ref{sec:eval}. However, given the computation and memory resource constraints of the machine on which we train our models, it is not feasible to always increase the forecasting window size to fit the increasing-size workloads. Moreover, we observe there are a large number ($\sim 17500$) of small templates with fewer than $25$ queries per day. It is inefficient to train a large number of per-template models for all the small templates. To improve the time and storage efficiency and deal with the huge templates, we propose to \cutNpack\ the templates into bins according to the model forecasting window size, the volume of templates, and the target applications. Based on the new bins, we adjust the pre-template model to the pre-bin model, \ie learn each model to forecast future queries for all the templates in the next time interval for each bin. We now describe the \cutNpack\ approach.


%Based on our observation, the recurrent templates have a stable number of queries per day. Thus we use the average number of queries per day to approximate the number of queries in the next day. Given the prediction window size $m$ and the average number of queries $\sigma_i$ per day for each template $i$, we group the templates into one bin, or divide one large template into separate bins, so that one prediction $m$ can cover the prediction for the next time interval for all the templates in a bin: $m \geq \sum_{i \in c_j} \sigma_i, \forall c_j$. Specifically, \textbf{Cut:} We cut the big templates into smaller time-interval bins so that one forecasting can cover the next time-interval. For example, the original observation time interval is one day. For a large template, we can divide a template into two sub-templates with the AM and PM time frames, or divide it into three sub-templates with smaller time intervals 0AM-8AM, 8AM-16PM, 16PM-12AM, \etc so that the forecasting window size can cover the sub-templates. \textbf{Pack:} We pack the small templates into larger volume bins to reduce the number of models to train and improve the training efficiency. We solve the bin-packing problem by greedily packing more templates as possible as long as one forecasting can cover the next interval queries in a bin. We show the detail of the \cutNpack\ in Algorithm~\ref{algo:clustering}. 



%Another large-volume issue is the prediction volume problem. Since our target application is view selecting, which is performed at a daily frequency. It is required that our models can predict one day volume's future queries at a time. This corresponds to $\sim 10,000 / 43,000 / 44,000$ queries per day for WT / SCOPE / BusTracker. It is difficult to build such a forecasting model to predict such a large volume at a time. To solve this challenge, \sys\ first proposes to train one model to predict for one template, and later proposes to cluster various workloads based on the workload features and adjust the pre-template model to the pre-cluster model to improve model efficiency. The per-template model is sufficient to solve the next-k query forecasting problem for small size workload. However, given the long query traces and a large number of templates in the real workloads (Table~\ref{tab:4statistics}), it is not efficient and not scalable to build and manage each model for each template. To further improve the time and storage efficiency, we propose to \cutNpack\ the templates into bins according to the capacity of models, volume of templates, and the target applications. Based on the new bins, \sys\ is able to adjust the pre-template model to the pre-cluster model, \ie learn each model to forecast for all the templates in one bin, thus reducing the total number of models to train and maintain and improve model efficiency. Now we discuss our \cutNpack\ algorithm. 


%Taking view selection as an example target application, it is required that the forecaster predicts all the future workloads that are needed by the next view selection interval. A common interval example to perform view selection is one day~\cite{}, and it is required that the models can predict all the next day's queries by the end of today before applying view selection and future queries come. To make \sys\ practical to view selection, we design our template distribution method based on the prediction window size of the models and the average numbers of queries of the templates, to both make the best of ML models capacity and fulfill the practical requirement.


%Based on our observation, the recurrent templates have a stable number of queries per day. %study in Section~\ref{sec:motivation}, the daily templates are the majority of the workload, and they have a very stable number of queries per day \todox{need to add this part in Sec 2} %\yuanyuan{Do you think we should consider building a model to predict the number of queries in the future time window for a template, and use that as the input for Algorithm 1 when deciding how to cut and pack tempates?}. 

After cutting and packing templates into bins, we now adapt the per-template models into per-bin models to solve the next-$\Delta t$ forecasting problem. We still use the \sysModel as the forecasting models, but have to make the following adaptations:

\squishlist
\item \textbf{The feature map} is more complex for a per-bin model, since it includes queries from all templates or sub-templates within a bin, rather than just one template. To account for multiple templates within each bin during featurization, it is necessary to include the template ID as a feature and the feature map must also encompass the parameter values from all templates within the bin.

\item 
\textbf{The forecasting task} becomes more challenging when modeling a mixed time-series pattern of various templates in a bin, as opposed to the pattern of a single template. The per-bin model must accurately forecast the template ID and all parameter values within the bin, to ensure that the predicted query can be correctly reconstructed with the appropriate template and parameter values.

%\item \textbf{The online feedback loop} is also improved. It is crucial to not only monitor model accuracy, fine-tune models, and detect new and inactive templates, but also to keep track of the size of each template. If the total size of templates exceeds the bin capacity, it becomes necessary to re-adjust the assignment of templates to bins and re-train the models for changed bins. 
\squishend

%With template \cutNpack, we adjust the per-template models to per-bin models by adapting the following aspects: (1) In preprocessing, we first \cutNpack\ the templates and build one feature map for each bin. (2) Instead of using one feature map to encode one template, we expand the feature map to encode all the attributes of all the templates in a bin. (3) We include the template ID so that the model can also forecast which template ID will come next in a bin. (4) When reconstructing the forecasted query, we refer to the template context by the template ID, and then fill the corresponding parameters into the template. %When constructing the feature map, if one attribute appears in the template, the featurization is the same as discussed in Section~\ref{sec:featurization}. Otherwise we set it as a special categorical value $\$$, as shown in Figure~\ref{fig:per_cluster_temp2}
%We deploy the per-bin models to solve the next time interval forecasting problem. We identify the forecasted queries for the next time interval by the forecasted arrival time.


%\hanxian{Need to discuss the algorithm name}
\begin{comment}
\begin{algorithm}
\caption{Template \cutNpack\ Algorithm}
\label{algo:clustering}
\begin{algorithmic}[1]
\State Input: models prediction window size $m$, the average number of queries $\sigma_i$ per day for each template $i$ in a descending order. $\sigma_{min} = \min(\sigma_i)$. The final packs set $C=\emptyset$. The temporary pack set $C_{temp}=\emptyset$.
\For {template $j$ in all templates}
    \If {$\sigma_j > m$}
        \State \textcolor{gray}{\# cut the large templates}
        \State divide template $j$ equally into $\lceil\frac{\sigma_j}{m}\rceil $ packs $c_{j}^1, ...,c_j^{\lceil\frac{\sigma_j}{m}\rceil}$
        \State $C = C \cup \{c_{j}^1, ...,c_j^{\lceil\frac{\sigma_j}{m}\rceil}\} $
    \Else
        \State \textcolor{gray}{\# pack the small templates}
        \State $Flag_{clustered} = 0$
        \For {$c_k $ in $C_{temp}$}
            \If {$Capacity(c_k) \geq \sigma_j $ }
                \State \textcolor{gray}{\# find the first-fit bin}
                \State $c_k = c_k \cup j$, $Capacity(c_k) = Capacity(c_k) - \sigma_j$
                \If {$Capacity(c_k) < \sigma_{min}$}
                \State $C = C \cup c_k, C_{temp} = C_{temp}-c_k $
                \EndIf
                \State $Flag_{clustered} = 1$, break
            \EndIf
        \EndFor
        
        \If {$Flag_{clustered} == 0$}
            \State \textcolor{gray}{\# otherwise allocate a new bin}
            \State New a pack $c_{new}=\{j\}$
            \State set $Capacity(c_{new})=m - \sigma_j$ 
            \If {$Capacity(c_{new}) < \sigma_{min}$}
                \State $C = C \cup c_{new}$
            \Else
                \State $C_{temp} = C_{temp} \cup c_{new}$
            \EndIf
        
        \EndIf
    
    \EndIf

\EndFor
\State $C = C \cup C_{temp}$
\State Output: the template pack set $C, s.t. m \geq \sum_{i \in c_k} \sigma_i, \forall c_k \in C$
\end{algorithmic}
\end{algorithm}
\end{comment}

\begin{comment}
\begin{figure}[ht!]
  \centering
  \includegraphics[width=\linewidth]{figure/per_cluster_temp2.pdf}
  \caption{New templatization adapted to per-cluster model.}
  \label{fig:per_cluster_temp2}
\end{figure}
\end{comment}

After forecasting queries for all bins, we collect results from all the per-bin models and sort-merge the queries based on the predicted arrival time. From per-template models to per-bin models, \sys\ is able to reduce the number of models by up to $23 \times$ as shown in Table~\ref{tab:estimatedPerModel} in our evaluation, and thus reduce the training and testing time and model storage overhead significantly. %Lin et al.~\cite{ma2018query} proposes to cluster the templates by semantics (e.g., the tables that it accesses) and similar arrival rate. In our study, we found the best packing methods vary case by case, depending on the workloads and the applications. Thus we design the template packing as a plug-in manner and users are able to customize their packing methods.

%\tar{My meta-comment for the whole of section 6 is that it seems a bit rushed. Perhaps, we want to explain in more detail 6.1 and 6.2 if not more formally (algorithm). This is also an important section compared to related work.}%\hanxian{TODO: finish a rewrite on S6, need reviews and comments}


\begin{comment}
\begin{table}[ht]
   \caption{The reduction rate of the number of models to train after performing template \cutNpack.}
  \label{tab:reduction}
  \resizebox{0.9\linewidth}{!}{
  \begin{tabular}{c|c|c|c|c}
    \hline
    & WT & SCOPE & BusTracker& MSSales\\
     \hline
    \# per-template models &2157 &168197 &258 &1143 \\
    \# per-bin models & 19 & 7716 & 50 &1\\
    \hline
    reduction rate & \textbf{113.5} & \textbf{21.8} & \textbf{5.16} & \textbf{1143}\\
  \hline
\end{tabular}}
\end{table}
\end{comment}



%For example, in our experiment, we found it is suitable for WT and SCOPE to cluster the templates by the same set of tables that the template access. For BusTracker, it is more feasible to cluster the templates by the similar query text (with only different lengths of IN Clause predicates). 




==> outline.tex <==
•	Some micro-experiments for motivation and analysis.
    	How off are the views if we do not do forecasting.
    	Why do we think we can do forecasting.

•	What patterns exist in the workloads we looked at? Can we characterize a few and discuss them with examples? (See the paper from CMU to understand how they do it).

•	Baselines:
    o	What could be a non-ML baseline. E.g., selecting based on frequency. Crystal sounds like a good baseline too.
    o	Simple ML baselines: Random Forest model?
    o	Explain why not they work. 

•	Templatization

•	Explain Per Template Model
    o	Pre-processing.
    o	Featurization and model.
    o	Why our modeling is novel.
    o	What are the issues without Per Template model.

•	Explain Per Input/Cluster Model

•	Explain how we are addressing Hard-To-Forecast Attributes
    o	How to we detect them.
    o	What do we do those attributes.

•	What optimizations we perform, e.g., to handle large number of attributes, etc. 

•	Parameter tuning if any

•	Workload characterization and summary

•	Application specific preprocessing

•	Incremental training 

•	Possible DB applications

•	Experiments.
o	Explain what metrics we are using and why.
o	Improvement on performance after view selection (pick any view materialization technique) when the input workload is selected using 
    	no forecasting
    	some heuristic technique (e.g., frequency based)
    	forecasting (results of our Per Input Model)
o	How the different forecasting techniques compare on accuracy vs storage vs training time. Methods to compare could be: 
    	No forecasting
    	Per Template Random Forest Model
    	Per Template Our Model
    	Per Input Model (No OPT)
    	Per Input Model (Full OPT)
o	Sensitivity analysis
    	Varying training window
    	Varying test window
    	Size of model
    	Effects of other optimizations



==> response-sigmod2024/header.tex <==
\graphicspath{{img/}}
%\usepackage{minted}
\usepackage{array}
%%\usepackage{lmodern}
\usepackage{amsmath}
%\usepackage{algorithmic}
%\usepackage[ruled,vlined]{algorithm2e}
\usepackage{pgfplots,pgfplotstable}  
\usepackage{booktabs}
\usepackage{balance}
\usepackage{multirow}
\usepackage{clipboard}
\usepackage{xcolor}
\usepackage{balance}

\usepackage{enumitem}
\usepackage{listings}
\definecolor{Keyword}{HTML}{0000ff}
\definecolor{KeywordType}{HTML}{2b91af}
\definecolor{String}{HTML}{a31515}

\lstdefinestyle{sql}{
	language=SQL,
	showspaces=false,
	basicstyle=\linespread{0.5}\small\ttfamily,
	numbers=none,
	xleftmargin=0em,
	numbersep=6pt,
	keywordstyle=\color{Keyword},
	stringstyle=\color{String},
	morekeywords={IF,BULK,PROCEDURE},
	classoffset=1, % type keyword highlighting
	keywordstyle=\color{KeywordType},
	classoffset=2, % sp1 keyword highlighting
	morekeywords={CleanAndAppendSalesHistory},
	keywordstyle=\color{mypurple},
	classoffset=3, % sp2 keyword highlighting
	morekeywords={SyncNewSales},
	keywordstyle=\color{darkgreen},
	escapeinside = {(*@}{@*)},
    escapechar=!
}

\newcommand{\todo}[1]{{\color{red}{TODO: }{#1}}}


\newcommand{\notdone}{ \noindent{\color{red}\fbox{\bfseries\sffamily\scriptsize{NOT DONE}}}}
\newcommand{\inprog} {\noindent{\color{blue}\fbox{\bfseries\sffamily\scriptsize{IN PROGRESS}}}}
\newcommand{\done} {\noindent{\color{darkgreen}\fbox{\bfseries\sffamily\scriptsize{DONE}}}}
%\newcommand{\done} {}



%\pgfplotsset{compat=newest}

\definecolor{darkgreen}{rgb}{0.0, 0.5, 0.0}
\newcommand{\system}{\texttt{QO-Advisor}\xspace}
\newcommand{\mynotemed}[1]{\par\noindent\colorbox{pink}{\parbox{\linewidth}{#1}}}
\newcommand{\mysimplenote}[1]{{#1}}
\newcommand{\mynote}[1]{\par\noindent\colorbox{lightgray}{\parbox{\linewidth}{#1}}}
\newcommand{\stitle}[1]{\vspace{0.5ex}\noindent{\bf #1}}

\newcommand{\AAG}[1]{\textcolor{purple}{\mynote{AA:~#1}}}
\newcommand{\aag}[1]{\textcolor{purple}{\mysimplenote{[AA:]~#1}}}
\newcommand{\AG}[1]{\textcolor{cyan}{\mynotemed{AG:~#1}}}
\newcommand{\ag}[1]{\textcolor{cyan}{\mysimplenote{[AG:]~#1}}}
\newcommand{\JCR}[1]{\textcolor{red}{\mynote{JCR:~#1}}}
\newcommand{\jcr}[1]{\textcolor{red}{\mysimplenote{[JCR:]~#1}}}
\newcommand{\rr}[1]{\textcolor{brown}{\mysimplenote{[RR:]~#1}}}
\newcommand{\cc}[1]{\textcolor{magenta}{\mysimplenote{[CC:]~#1}}}
\newcommand{\af}[1]{\textcolor{darkgreen}{\mysimplenote{[AF:]~#1}}}



%--- Terminology ---
%\newcommand\vldbpagestyle{plain} 
%\newcommand {\sys}{\textsc{Sibyl}\xspace}
%\newcommand {\sysModel}{\textsc{Sibyl-LSTMs}\xspace}
%\newcommand{\cutNpack}{Cut-and-Pack\xspace}
\newcommand{\sklearn}{\textsc{Scikit-Learn}\xspace}
\newcommand{\numpy}{\textsc{Numpy}\xspace}
\newcommand{\matplotlib}{\textsc{Matplotlib}\xspace}
\newcommand{\pandas}{\textsc{Pandas}\xspace}
\newcommand{\scipy}{\textsc{Scipy}\xspace}
\newcommand{\seaborn}{\textsc{Seaborn}\xspace}
\newcommand{\theano}{\textsc{Theano}\xspace}
\newcommand{\nolearn}{\textsc{NoLearn}\xspace}
\newcommand{\keras}{\textsc{Keras}\xspace}
\newcommand{\nimbusml}{\textsc{NimbusML}\xspace}
\newcommand{\tensorflow}{\textsc{TensorFlow}\xspace}
\newcommand{\mxnet}{\textsc{Mxnet}\xspace}
\newcommand{\os}{\textsc{Os}\xspace}
\newcommand{\cv}{\textsc{OpenCV}\xspace}
\newcommand{\PIL}{\textsc{Pillow}\xspace}
\newcommand{\torch}{\textsc{PyTorch}\xspace}
\newcommand{\caffe}{\textsc{Caffe}\xspace}
\newcommand{\nltk}{\textsc{NLTK}\xspace}
\newcommand{\re}{\textsc{Regular Expression}\xspace}
\newcommand{\pylab}{\textsc{Pylab}\xspace}
\newcommand{\statsmodels}{\textsc{StatsModels}\xspace}
\newcommand{\requests}{\textsc{Requests}\xspace}
\newcommand{\xgboost}{\textsc{XGBoost}\xspace}
\newcommand{\gensim}{\textsc{Gensim}\xspace}
\newcommand{\tqdm}{\textsc{Tqdm}\xspace}
\newcommand{\sqlalchemy}{\textsc{SQLAlchemy}\xspace}
\newcommand{\bs}{\textsc{bs4}\xspace}
\newcommand{\lasagne}{\textsc{Lasagne}\xspace}
\newcommand{\dataframe}{\textsc{DataFrame}\xspace}
\newcommand{\plotly}{\textsc{Plotly}\xspace}
\newcommand{\selenium}{\textsc{Selenium}\xspace}
\newcommand{\csn}{\textsc{cs231n}\xspace}
\newcommand{\torchvision}{\textsc{TorchVision}\xspace}
\newcommand{\hpy}{\textsc{\textsc{H5py}}\xspace}
\newcommand{\gym}{\textsc{\textsc{Gym}}\xspace}
\newcommand{\lgbm}{\textsc{\textsc{LightGBM}}\xspace}
\newcommand{\imblearn}{\textsc{\textsc{Imblearn}}\xspace}
\newcommand{\csv}{\textsc{\textsc{Csv}}\xspace}
\newcommand{\json}{\textsc{\textsc{Json}}\xspace}
\newcommand{\zipfile}{\textsc{\textsc{ZipFile}}\xspace}
\newcommand{\gzip}{\textsc{\textsc{Gzip}}\xspace}
\newcommand{\sqlite}{\textsc{\textsc{SQLite3}}\xspace}
\newcommand{\psycopg}{\textsc{\textsc{Psycopg3}}\xspace}
\newcommand{\pymysql}{\textsc{\textsc{PyMySQL}}\xspace}
\newcommand{\timepkg}{\textsc{\textsc{Time}}\xspace}

\newcommand{\pudf}{pandas\_udf}
\newcommand{\sparksideudf}{client-side UDF\xspace}
\newcommand{\companyname}{CompanyX\xspace}
\newcommand{\rfscore}{\textit{RF Scoring}\xspace}
\newcommand{\parquetproj}{Apache Parquet\xspace}
\newcommand{\parquetcon}{\textit{Parquet}\xspace}
\newcommand{\socketscon}{\textit{Sockets}\xspace}
\newcommand{\arrowflightcon}{\textit{Arrow Flight}\xspace}
\newcommand{\arrowflightproj}{Arrow Flight\xspace}
\newcommand{\mlflowcon}{\textit{MLflow}\xspace}
\newcommand{\webservcon}{\textit{Web Server}\xspace}
\newcommand{\mlflowproj}{MLflow\xspace}
\newcommand{\azfabbrev}{AZF\xspace}

\newcommand{\regserv}{\textit{Registration Service}\xspace}
% next two got combined.
\newcommand{\udfsvc}{\textit{Data Processing System}\xspace}
\newcommand{\dataeng}{\textit{Data Processing System}\xspace}
\newcommand{\cudfsvc}{\textit{Containerized UDF Service}\xspace}
\newcommand{\cm}{\textit{Container Manager}\xspace}
\newcommand{\cudfs}{\textit{Containerized UDFs}\xspace}
\newcommand{\execeng}{\textit{Execution Engine}\xspace}

\newcommand{\limit}[1]{\textbf{$\textrm{L}$#1}\xspace}
\newcommand{\checkgreen}{\textcolor{teal}{\textbf{\checkmark}}}
\newcommand{\redex}{\textcolor{red}{\textit{$\times$}}}
\newcommand{\gh}{\textsc{GitHub}\xspace}
\newcommand{\tlc}{\textsc{ML.net}\xspace}
\newcounter{enum}
\newenvironment{packed_enum}{
	\begin{list}{\textbf{(\arabic{enum})}}{
			\setlength{\itemsep}{0pt}
			\setlength{\parskip}{0pt}
			\setlength{\labelwidth}{-4pt}
			\setlength{\leftmargin}{0pt}
			\setlength{\itemindent}{0pt}
			\usecounter{enum}}
	}{\end{list}}
\newcounter{reviewer}
%\setcounter{reviewer}{0}
\newcounter{point}[reviewer]

\newenvironment{point}[1]
{\refstepcounter{point} \medskip \noindent {\textbf{#1:} }\it \color{teal}}
{\par }

\newcommand{\shortpoint}[1]{\refstepcounter{point}  \bigskip \noindent 
	{\textbf{Reviewer~Point~\thepoint} } ---~#1\par }

\newenvironment{reply}
{\medskip \noindent \begin{sf}\  }
{\medskip \end{sf}}

\newenvironment{response}
{\medskip \noindent \begin{sf}\textbf{Response:}\  }
{ \end{sf}}

\newenvironment{changes}
{\medskip \noindent \textbf{Changes to the paper:}\ \color{blue} }
{\medskip }

%\newcommand{\changes}[1]{\noindent\textbf{Changes made in the paper.} \textcolor{blue}{#1}}


==> response-sigmod2024/response.tex <==
%\documentclass[sigconf, nonacm]{../acmart}

%\include{header}
%\usepackage{afterpage}

%\begin{document}

% \title{Response to Reviewer Comments\\ \sys: Forecasting Time-Evolving Query Workloads}

% \title{Response to Reviewers' Comments}
% \maketitle

%\balance

\twocolumn[\section*{Response to Reviewers' Comments}]

We thank the reviewers for their critical assessment and suggestions that helped us improve our paper. We addressed all comments in the revised version and used {\color{blue} blue} font to highlight new/updated text. Below we summarize the major changes and then provide responses to each of the specific comments and indicate the corresponding changes in the paper. 

\subsection*{META-REVIEWER}

\begin{point}{M1}%\notdone
Major Revision Items:

\begin{itemize}[leftmargin=*]
    \item Add the clarifications requested by R1 (see Q14 and Q17).
    \item Add the future work, overhead, and use case discussions requested by R2 (see Q14).
    \item Add the experiments listed by R3 (see Q14).
\end{itemize}
\end{point}

\begin{response}
We thank the reviewers for providing feedback and giving us the chance to incorporate their comments into the revised version. We feel this endeavor definitely helped to improve the paper! We have addressed all the listed revision items (details see below).
\end{response}

\noindent\textbf{\revision{Summary of Major Changes:}}
\revision{
\begin{packed_enum}
    \item We added comparison to two additional ML models, an adapted Random Forest (suggested by Reviewer 1), and a Transformer based decoder-only model (suggested by Reviewer 3) in Section~\ref{subsec:compofmodels}.
    \item We added index selection as another application for \sys in Section~\ref{sec:eval_index_selection} (suggested by Reviewers 1 \& 2).
    \item We added one more baseline, TEALED~\cite{tealed}, in Section~\ref{sec:baselines} and compare and contrast event-based forecasting~\cite{8781017} vs time-based forecasting (\sys) in related work (Section~\ref{sec:related}) (both suggested by Reviewer 3).
    \item We added the prediction overhead of \sys in Section~\ref{sec:efficiency} (suggested by Reviewer 1) and the overhead comparison to existing works in Section~\ref{sec:baselines} (suggested by Reviewer 2).
    \item We added comparison with existing works for view recommendation and the newly added index selection applications in Section~\ref{sec:eval_applications} and Section~\ref{sec:eval_index_selection} (suggested by Reviewer 2).
    \item We changed the History method for view selection to include 7 days of queries instead of just 1 day in Section~\ref{sec:eval_applications} (suggested by Reviewer 3).
    \item We added experiments on the effect of bin size in Section~\ref{sec:effect_bin_size} (suggested by Reviewer 1 \& 3).
    \item We added discussion of fine-tuning overhead in Section~\ref{sec:eval_fineTunning} (suggested by Reviewer 1).
\end{packed_enum}
}

\section*{Reviewer 1}

\begin{point}{O6}%\notdone
\textbf{Before Author Feedback}: It seems that a fundamental assumption made in the template cutting technique is that the sub-templates preserve the same time series pattern as the original template. But I'm concerned that this assumption might be too strong. For example, if the sub-template is cut at every hour, but the original template has a periodic pattern for every 50 minutes. Then how the sub-template preserve the pattern in the original template?\\
\textbf{After Author Feedback}: The authors cite a new paper ([52]) to justify the assumption on the sub-template patterns. I think they should expand on that in the paper and add additional explanations and clarifications to help the audience intuitively understand why the assumption is valid.
\end{point}

\begin{comment}
\begin{response}
Thanks for the suggestion! We added the explanation and clarification.
\end{response}
\end{comment}

\begin{changes}
Thanks for the suggestion! We added the explanation and clarification in the 2nd paragraph in Section~\ref{sec:cut}.
\end{changes}

\begin{point}{O4}%\notdone
\textbf{Before Author Feedback}: For the RF model, can we have all features from $q_{n-k+1}$ to $q_{n}$ as input and all $q_{n+1}$ to $q_{n+k}$ as output? It seems unfair to compare RF that predicts a single timepoint versus LSTM/SIBYL-LSTM that uses the entire sequence of k timepoints as input.\\ 
\textbf{After Author Feedback}: My question is what if we use all the values from $q_{n-k+1}$ to $q_{n}$ as input and predicts $q_{n+1}$ to $q_{n+k}$ together as output? Would RF perform better with this featurization? I think this might be a fair comparison since LSTM/SIBYL-LSTM uses the entire sequence of k time points as input as well.
\end{point} %\tar{we can cut this comment short to make space, we only need from "my question" onwards.}

\begin{comment}
\begin{response}
We adapt RF to use all the values from $q_{n-k+1}$ to $q_{n}$ as input by concatenating all the parameters in $q_{n-k+1}$ to $q_{n}$ into a single input vector, and get all parameters of $q_{n+1}$ to $q_{n+k}$ as output together. We refer such adaptation as RF+ and show the results in Section 9.3.1.
\end{response}
\end{comment}

\begin{changes}
We added the results of such adapted RF in Section~\ref{subsec:compofmodels}. We refer such adaptation as RF+.
\end{changes}


\begin{point}{O1}%\notdone
What's the definition of recurrent queries/template? Queries that appear more than once? That might be a too relax definition. For example, an ad-hoc queries may appear twice consecutively and never appear again.
\end{point}

\begin{response}
We have clarified the definition in the revision. Note that ad-hoc signals have little effect on model accuracy due to the dominance of frequent recurrent queries, which is also well observed in prior work~\cite{jindal2021production,alibaba,ma2018query,abebe2022tiresias,CrocodileDB,p-store}.%\rana{cite?}
\end{response}

\begin{changes}
We added concrete definition in Observation 1 of Section~\ref{sec:motivation} along with references to prior work that make similar observations. We also added statistic and observation of dominance of frequent recurrent queries in Observation 1 of Section~\ref{sec:motivation}.
\end{changes}


\begin{point}{O2}%\notdone
Similary, what is the definition of evolving template? If a template has 1000 queries but only two parameter combinations, is it still evolving?
\end{point}

\begin{response}
As defined in Observation 2 of Section~\ref{sec:motivation}, a recurrent template with at least one changing parameter value is an evolving template. A template with 1000 queries but only two parameter combinations is an evolving template, since how the parameter alternates between the two values could present time evolving pattern.
\end{response}

%\begin{changes}
%\end{changes}


\begin{point}{O3}%\notdone
Out of the four patterns shown in Figure 2, it seems that the only valuable prediction is the trending pattern (or the trending portion of the combination pattern)? The random pattern does not seem to be tractable and I'm not sure how much value there is to predict the periodic pattern since each period is the same (in other works, the workload is "static" as long as the workload window is larger than the period).
\end{point}

\begin{response}
While strictly periodic patterns are easily predictable, in practice multiple patterns are intertwined (e.g. Figure~\ref{fig:CommonPatterns}(c)), arrival rates may not be strictly regular (e.g., variations over weekdays vs. weekends), and parameters within the same query template differ in patterns, making naive forecasters insufficient (as shown in the results in Section~\ref{sec:eval}). %\tar{do we have an example of intertwined patterns from our workload that we can point to?}
\end{response}

%\begin{changes}
%\end{changes}


\begin{point}{O5}%\notdone
The techniques used in SIBYL-LSTM seems to be a straightforward application of encoder-decoder architecture with LSTMs. What are the technical challenges solved for SIBYL-LSTM?
\end{point}

\begin{response}
Our primary contribution lies in defining/modeling the problem of forecasting complete queries (Section~\ref{sec:Problem}), adapting ML techniques (feature representation, combining encoder-decoder with LSTMs, Section~\ref{sec:design-k}) for better accuracy, and improving scalability through template cutting and packing (Section~\ref{sec:design-delta}). 
\end{response}

\begin{changes}
We modified the abstract, and added the clarification in the last paragraph of Section~\ref{sec:intor}.
\end{changes}


\begin{point}{O7}%\notdone
For the per-bin models, what is the adaption made to the model for the second challenge (the forecasting take becomes more challenging)?
\end{point}

\begin{response}
In Section~\ref{sec:design-delta}, we emphasize the proposed per-bin forecasting paradigm to solve the critical challenge of huge possible forecasting size as well as the efficiency and scalability issues of small templates. We mainly adapt the model input (featurization, template cutting and packing) to enable such forecasting adaptation. For model itself, we still use \sysModel since we found them sufficient to address the challenge of forecasting the mixed time-series patterns of various templates. %Other ML techniques such as Transformer-based models may be possible for the forecasting challenge, which is left as our future work. 

Moreover, we limit the bin size (total number of templates in a bin) to better control the trade-offs between model accuracy and efficiency. %We added results and discussions of the effect of bin size in Section~\ref{sec:effect_bin_size} and how we empirically selected the bin size for \sys.
The implications of bin size and its selection for \sys are discussed and detailed in Section~\ref{sec:pack} and Section~\ref{sec:effect_bin_size}, where we also present our results on empirically selecting the bin size. %for \sys.
\end{response}

\begin{changes}
We added a discussion on the bin size in Section~\ref{sec:pack} and an empirical study of this in Section~\ref{sec:effect_bin_size}.
\end{changes}


\begin{point}{O8}%\notdone
The model storage and training overhead seems to be really high even for the per-bin models. For example for system S, the training time is 685 h (28 days) and the storage overhead is 771 GB. Do the authors really spend a month training this model? And for the per-template model, do the authors train for a year (9344 h)?
\end{point}

\begin{response}
Models are indexed by template/bin id and only the required ones are loaded, so storage of 771GB is less concerning for our setting. The reported training time is “aggregated” over “all” templates/bins. We can reduce the elapsed time via parallelized training and compressing models.
\end{response}

\begin{changes}
We added clarification in the Experimental Setup of Section~\ref{sec:eval}, Section~\ref{sec:efficiency}, and Table~\ref{tab:estimatedPerModel}.
\end{changes}


\begin{point}{O9}%\notdone
What is the fine-tuning overhead when workload shifts?
\end{point}

\begin{response}
The average fine-tuning time per epoch is under 10s for a per-template model and 16s for a per-bin model, due to the smaller size of new observed data. In \sys, we limit the maximum number of fine-tuning epochs to 20. In our experiments, we found the fine-tuning convergences much faster than 20 epochs, which leads to only a few seconds of fine-tuning overhead.
\end{response}

\begin{changes}
We added the discussion on fine-tuning overhead in Section~\ref{sec:eval_fineTunning}.
\end{changes}


\begin{point}{O10}%\notdone
It would be good to show the benefit of SIBYL on either more applications (e.g., index selection) or more workloads (besides Sales).
\end{point}

% \begin{response} We added a new experiment on index recommendation using the Telemetry workload in Section~\ref{sec:eval_index_selection}.
% \end{response}

\begin{changes}
We added a new experiment on index recommendation using the Telemetry workload in Section~\ref{sec:eval_index_selection}.
\end{changes}


\begin{point}{O11}%\notdone
Is the "a few milliseconds" prediction overhead per model? Even though the prediction overhead is much smaller than training (which is expected), it is still important to know the total overhead to make the prediction for the entire workload over different $\Delta t$.
\end{point}

%\begin{response}
%\end{response}

%\begin{changes}
%We added the prediction times in the last paragraph of Section~\ref{sec:efficiency}.
%\end{changes}

\begin{response}
We would like to emphasize that none of the phases in \sys, including the prediction phase, is in the critical path of workload-based optimization application. Query prediction can be done offline to prepare the inputs for these applications to tune database performance. The models are indexed by their respective templates or bin ids. This allows us to load only the required models at the time of forecasting. As added in the last paragraph of Section~\ref{sec:efficiency}, the aggregate prediction time for all models are at most a few minutes. We can also parallelize the prediction process by employing multiple machines.
\end{response}

\begin{changes}
We added the aggregate prediction times in Section~\ref{sec:efficiency}. We also added some clarification in the last paragraph of Section~\ref{sec:overview}.
\end{changes}


\subsection*{Reviewer 2}

\begin{point}{O1}%\notdone
The workloads seem biased toward select queries. How common were DMLs and DDLs? What effect would this have on both the forecasting accuracy and performance benefits of applying Sibyl's forecasts?
\end{point}

\begin{response}
SIBYL primarily focuses on analytic workloads targeting workload-based optimization applications. While our techniques are general enough, we leave evaluation over DML and DDL as future work.
\end{response}

\begin{changes}
We added the clarification in the last paragraph of Section~\ref{sec:Problem}.
\end{changes}


\begin{point}{O2}%\notdone
The experimental section could be improved.

\begin{itemize}[leftmargin=*]
	\item Sibyl was only used vs other systems to determine accuracy. It would be nice to see it compared in terms of overheads, and in the view selection application. A geometric mean or summary of the results would also help.
	\item It would also be good to see Sibyl used for more applications especially eg cloud elasticity or index selection.
\end{itemize}
\end{point}

%\begin{response}
%\end{response}

\begin{changes}
\begin{itemize}[leftmargin=*]
\item We added the prediction overhead comparison in Table~\ref{tab:CompRelated}. 

\item In the view recommendation experiment detailed in Section~\ref{sec:eval_applications}, we included a comparison with Q-Learning+ and QueryBot5000+. 
Additionally, we changed the view recommendation on the history workload to cover 7 days of queries instead of 1 day. 
\item We also added a new experiment focusing on index selection in Section~\ref{sec:eval_index_selection}. 
\end{itemize}

%\todo{Hanxian will fill the numbers in Table 10 later.}  %\todo{Should we also compare the overheads of \sys against Q-learning and Querybot?}
\end{changes}



\subsection*{Reviewer 3}

\begin{point}{O1}%\notdone
\textbf{Before Author Feedback}: The proposed method is not practical because the large number of per-template models or per-bin models will cost a lot of storage and GPU resources (training and predicting, see more detail in O12). The paper builds a model for each query template instead of build a global model. However, there are a lot of query templates in real-world workloads. The model number is still large even with packing templates into bins, shown in Table 8.\\
\textbf{After Author Feedback}: Please add experiments to evaluate the model performance of varying number of per-bin models. In another word, select the best size of bin of per-bin model.
\end{point} %\tar{this comment can be made shorter too, we only need after author feedback maybe}

\begin{response}
A global model is less optimal in practice: (1) has poor accuracy due to packing of many complex time-series patterns with different evolving parameters. (2) requires larger training data and is more expensive to train. (3) infeasible due to limited GPU resources and large next-t forecasting window size, e.g., ~200K queries in next day for Telemetry workload. In contrast, adaptive per-bin SIBYL models achieve both better scalability and accuracy. Similar observations have also been made in prior works [29, 43, 49]. 

Regarding practicality, please see our response and changes for Reviewer1.O8.

The implications of bin size and its selection for \sys are discussed and detailed in Section~\ref{sec:pack} and Section~\ref{sec:effect_bin_size}, where we also present our results on empirically selecting the bin size. 

%\todo{Add experiments on bin size.}
\end{response}

%for \sys.

\begin{changes}
We added a discussion on the bin size in Section~\ref{sec:pack} and an empirical study of this in Section~\ref{sec:effect_bin_size}. We also highlighted the limitation of global model in the first paragraph of Section~\ref{sec:design-k}.
\end{changes} %\tar{we may also want to clarify in the paper why a global model is not preferable.} 
%\rana{I believe this is already highlighted in Section 5.}


\begin{point}{O5}%\notdone
\textbf{Before Author Feedback}: Really need encoder-decoder architecture? The paper did not discuss the significance of encoder-decoder architecture and why choose this architecture. Can decoder-only architecture performance the same?\\
\textbf{After Author Feedback}: Add experiments to compare a transformer method rather than leaving it to the future work.
\end{point}

\begin{response}
The encoder captures inter-dependencies among multiple variables better than vanilla LSTM as we have explained in the 3rd paragraph of Section~\ref{sec:templatemodels}.

Transformer-based models are indeed promising for our setting. As suggested by the reviewer, we have now added an empirical evaluation on the Transformer based Decoder (denoted by TRF) in the second paragraph of Section~\ref{subsec:compofmodels}.
We find that TRF attains a slightly better accuracy than \sysModel (Table~\ref{tab:CompMoreModels}). However, we observe that TRF requires $18.2\times$ more training time and $4.4\times$ more model storage overhead. While there could be potential optimization to reduce these overheads for TRF, our observation is that  \sysModel and TRF are comparable in accuracy, with \sysModel offering a better trade-off between accuracy and efficiency.

We leave a more detailed comparison of these trade-offs and the potential optimization of TRF as a future work. We want to clarify (as highlighted in the last paragraph of Section 1) that the primary contribution of \sys is not the development of new ML algorithms, rather it lies in leveraging these models for 
 forecasting \textit{entire} query statements and their adaptation for better accuracy and scalability. Our study shows that \sysModel for \sys strikes a good balance between accuracy and efficiency.

\end{response}

\begin{changes}
We added experiments on a Transformer-based model in Section~\ref{subsec:compofmodels} and clarification in Section 1 on the primary focus of \sys as summarized above.
\end{changes}

\begin{point}{O8}%\notdone
\textbf{Before Author Feedback}: Poor baselines in experiment. The three baselines history-based, Random Forest, and Vanilla LSTM is not enough as baselines. More baselines from previous works are needed, e.g.,~\cite{tealed,8781017}.\\
\textbf{After Author Feedback}: Add experiment with more baselines in addition to QueryBot5000 and Q-Learning.\\
\end{point}

\begin{response}
Thanks for pointing out these two related works (\cite{8781017,tealed}).

The paper \cite{tealed} utilizes a combination of time-sensitive empirical mode decomposition (EMD) and
auto LSTM encoder-decoder to forecast resource utilization and query arrival rates for DBMSs. Like QueryBot5000, it does not predict query statements. Similar to the adaptation to QueryBot5000 baseline, we adapt it to predict query statements and show the results in Table~\ref{tab:CompRelated}.

Based on the observation that database workloads are correlated with real-world events, \cite{8781017} forecasts future workloads, presuming knowledge of the real-world events that will occur in the future, by matching them to similar events in the history. This work targets at event-based forecasting, instead of time-based forecasting, which \sys focuses on. Such ideas seem plausible for databases where workloads depend on specific events and we know/track events in time (e.g., DB underlying CMT or those behind sports websites). However, it's not feasible for us to empirically compare with this approach. We do not know the real-world events in the applications that triggered the workload we are evaluating. The problem setup and targeted scenarios are different/orthogonal and can't be aptly compared. 
%we can cut the next line} Note that our solution is also more general since we don't depend on events and a ML model can forecast accurately even if there is some irregularity in arrival times.
\cite{8781017} also does not capture evolution, i.e., they can't predict queries unseen in history.

\end{response}

\begin{changes}
We compared and contrasted \sys with these two works in Section~\ref{sec:related}, and added empirical results on \cite{tealed} in Section~\ref{sec:baselines}.
%\todo{Add experiment}
\end{changes}

\begin{point}{O9}%\notdone
\textbf{Before Author Feedback}: Inappropriate usage of materialized views selection algorithm in Session 9.5. The paper train a model using 2237 Sales queries over 20 consecutive days. But only select views on one day (preceding day or succeeding day) queries. Actually, for materialized views selection, queries of more days should be used to search the recurrent queries. Moreover, many materialized view definitions do not vary over date because they are often GROUP BY date. Experiment design on materialized views selection should be improved.\\
\textbf{After Author Feedback}:  Add an experiment recommending views based on multiple days’ queries.
\end{point}

%\begin{response}
%\end{response}

\begin{changes}
We changed the view recommendation on the history workload to cover 7 days of queries instead of 1 day in Section~\ref{sec:eval_applications}. We also added comparison to Q-Leanrning+ and QueryBot5000+ in the view recommendation experiment. 
\end{changes}

\begin{point}{O2}%\notdone
The query featurization method is too simple and unreasonable. Featurization is important in query prediction problems, but the paper used inappropriate featurization method for categorical, string, char, and set types. First, the paper handles string and set value as categorical types, and assign an identical integer value to each category, which means they assign size relationship between two categorical values, that is wrong. Instead, the one-hot vector should be used to represent categorical types. I think the paper does not use one-hot vector because there are extremely large number of different values, resulting in super large feature vector.
\end{point}

\begin{response}
We apply a widely used feature hashing to assign integers to categorical parameters without explicitly assigning size relationships between two categorical values. We choose it as an alternative to one-hot encoding to deal with the challenge of high cardinality categorical features as the reviewer also mentioned. Featuring hashing is able to handle a new category by assigning an integer and avoiding adding new columns in the feature map.
\end{response}

\begin{changes}
We added clarification in Section~\ref{sec:queryFeatureVector}.
\end{changes}


\begin{point}{O3}%\notdone
The query featurization method cannot generate new string because the method collects all possible values from the training data (history query). However, new values will appear and be a significant part of time evolving workloads. Moreover, in Session 7 feedback loop, when fine-tuning the model, the paper did not discuss how to extend the vocabulary of parameter values when collecting new training data. The generation and training of new parameter values should be considered or discussed more.
\end{point}

\begin{response}
During fine-tuning, SIBYL extends vocabulary of parameter values by assigning new categorical values with hashing values.
\end{response}

\begin{changes}
We added clarification in Section~\ref{sec:feedbackloop}.
\end{changes}


\begin{point}{O4}%\notdone
The paper packs templates into bins, to reduce the number of models, but did not give a proper way to adapt the per-template models into per-bin models. Packing templates will result in critical problems such as, putting different types (e.g., numerical and categorical) of features in the same position of vector, mixed time-series pattern. I do not think including the template id in the feature vector can solve these problems.
\end{point}

\begin{response}
We assign unique identifiers and positions to each of the parameters from various templates in the feature vector e.g., a bin containing two templates with 3 and 2 parameters respectively, will have a feature vector with 5 parameters.
\end{response}

\begin{changes}
We added clarification in 
Section~\ref{sec:perbinmodel}.
\end{changes}

\begin{point}{O6}
Template Cutting (in session 6.2) method is unreasonable and will hurt the predict performance. The paper has a wrong assumption that the queries in a specific hour among days are recurrent. Actually, the appearance of a query or template could fall into random hours because of disturbance of many reasons. The template should be cut better or sampled.
\end{point}

\begin{response}
Template cutting adjusts intervals based on arrival rates of queries and prediction interval (not specific to 1 hour). We also added more explanation in Section~\ref{sec:cut}.
\end{response}

\begin{changes}
We added the explanation and clarification in the 2nd paragraph in Section~\ref{sec:cut}.
\end{changes}


\begin{point}{O7}%\notdone
The parameter values are predicted well in Figure 9, but the names of the three parameters are ignored. We do not know why they are predicted well and whether these parameters are useful. Please add more information.
\end{point}

%\begin{response}
%\end{response}

\begin{changes}
For privacy reasons, we are unable to provide the exact names of these parameters, but we have now added more information about them in Section~\ref{sec:individual_acc}.
\end{changes}

\begin{point}{O10}%\notdone
In session 8 effectiveness measurement, the precision evaluation of the prediction depends on the maximum bipartite matching of G. However, this measurement did not take into consideration the order of the predicted queries, which is relatively important in time-series prediction problems. Moreover, the unpredictable parameters are ignored in measurement, which make the precision higher than the truth. The measurement function could be designed better.
\end{point}

\begin{response}
Predicting arrival of queries within a small-time window (e.g., 1h, 6h, 1day) is generally sufficient for our target applications (view recommendation, index selection, partitioning of tables, and determination of the MDC of tables), strict ordering is unnecessary. These applications generally look at all queries from a given window without considering their ordering. We report the prediction accuracy for all parameters including random ones in Section 9.1. Random parameters can’t be predicted. We believe the right approach is to be able to identify them and not apply any constraints on them (Section 8).
\end{response}

%\begin{changes}
%\end{changes}


\begin{point}{O11}%\notdone
The Cnt-diff ratio is reported in Table 7. The proposed method Sibyl-LSTMS is not always better than other methods (Random Forest, Vanilla LSTM). For example, when dataset Telemetry and k=500, Random Forest has Cnt-diff ratio as 0.04 but Sibyl-LSTMS has Cnt-diff ratio as 0.22 (worse). Please give more analyze on these results.
\end{point}

%\begin{response}
%\end{response}

\begin{changes}
We added more analysis in Section~\ref{sec:kmodelcomparision}.
\end{changes}


\begin{point}{O12}%\notdone
In 9.2.2, window size is set to 1000 to avoid the out of memory of GPU. Does it mean that one model prediction occupies one GPU? Therefore, it takes a lot of time to do the prediction for all per-template or per-bin models. But the total prediction time is ignored in 9.3.3 and Table 8. The total prediction time should be reported.
\end{point}

\begin{response}
Please see our response and changes for Reviewer1.O11.
%We would like to emphasize that none of the phases in \sys, including the prediction phase, is in the critical path of workload-based optimization application. Query prediction can be done offline to prepare the inputs for these applications to tune database performance. The models are indexed by their respective templates or bin ids. This allows us to load only the required models at the time of forecasting. As shown in the last paragraph of Section~\ref{sec:efficiency}, the aggregate prediction time for all models are at most a few minutes. We can also parallelize the prediction process by employing multiple machines.
\end{response}

%\begin{changes}
%We added the prediction times in Section~\ref{sec:efficiency}. We also added some clarification in the last paragraph of %Section~\ref{sec:overview}.
%\end{changes}

%\bibliographystyle{ACM-Reference-Format}
%\bibliography{sample}

%\end{document}
%\endinput

